Getting High: High Fidelity Simulation of High Granularity Calorimeters with High Speed

Accurate simulation of physical processes is crucial for the success of modern particle physics. However, simulating the development and interaction of particle showers with calorimeter detectors is a time consuming process and drives the computing needs of large experiments at the LHC and future colliders. Recently, generative machine learning models based on deep neural networks have shown promise in speeding up this task by several orders of magnitude. We investigate the use of a new architecture -- the Bounded Information Bottleneck Autoencoder -- for modelling electromagnetic showers in the central region of the Silicon-Tungsten calorimeter of the proposed International Large Detector. Combined with a novel second post-processing network, this approach achieves an accurate simulation of differential distributions including for the first time the shape of the minimum-ionizing-particle peak compared to a full GEANT4 simulation for a high-granularity calorimeter with 27k simulated channels. The results are validated by comparing to established architectures. Our results further strengthen the case of using generative networks for fast simulation and demonstrate that physically relevant differential distributions can be described with high accuracy.

==> version_0/1_ABSTRACT.tex <==
\begin{abstract}

Accurate simulation of physical processes is 
crucial for the success of modern particle physics.
However, simulating the development and interaction of particle showers with calorimeter detectors is a time consuming process and  drives the computing needs of large experiments at the LHC and future colliders. Recently, generative machine 
learning models based on deep neural networks have shown promise in speeding up this task by several orders of magnitude. We investigate 
the use of a new architecture --- the Bounded Information Bottleneck Autoencoder ---
for modelling electromagnetic showers in the central region of the Silicon-Tungsten calorimeter
of the proposed International Large Detector. Combined with a novel second post-processing network, this approach
%for the first time 
achieves an accurate simulation of differential distributions 
including for the first time  the shape of the minimum-ionizing-particle peak
compared to a full GEANT4 simulation for a high-granularity calorimeter with
27k simulated channels. The results are validated by comparing to established architectures. 
%and show the general applicability of the post-processing network.
Our results further strengthen the case of using generative networks for fast simulation and demonstrate that 
physically relevant differential distributions can be described with high accuracy.

%demonstrates the potential of using such networks for fast calorimeter simulation for ILD detector in the future and opens the possibility to complement current simulation techniques.

%We investigate the usage of Generative Adversarial Networks (GANs) and Bounded Information Bottleneck Autoencoder (BIB-AE) for modeling the electromagnetic showers in the context of proposed International Large Detector (ILD), in the central region of Silicon-Tungsten (Si-W) Electromagnetic Calorimeter. After successful completion of the training processes, the properties of synthesized showers are compared to the showers from a full detector simulation using Geant4. Our results demonstrates the potential of using such networks for fast calorimeter simulation for ILD detector in the future and opens the possibility to complement current simulation techniques.

\keywords{Deep learning \and Generative models 
\and Calorimeter \and Simulation \and High granularity \and 
GAN \and WGAN \and BIB-AE}
% \PACS{PACS code1 \and PACS code2 \and more}
% \subclass{MSC code1 \and MSC code2 \and more}
\end{abstract}

==> version_0/2_TEXT.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% INTRODUCTION
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{sec:intro}

Precisely measuring nature’s fundamental parameters and discovering new 
elementary particles in modern high energy physics is only made possible
by our deep mathematical understanding of the Standard Model
and our ability to reliably simulate interactions of these particles 
with complex detectors. While essential for our scientific progress,
the production and storage of these simulations is increasingly costly.
This cost is already a potential bottleneck at the LHC,
and the problem will be exacerbated by higher luminosity,
larger amounts of pile-up and more complex and granular detectors at the high-luminosity
LHC and planned future colliders. 
A promising way to accelerate the simulation is offered by generative machine learning models~\cite{CaloGAN2}. 
The present work focuses on simulating a very high-resolution calorimeter prototype with greater fidelity of
physically relevant distributions, paving the road for practical applications~\footnote{Implementations of
the network architectures as well as instructions to produce training data are available on \\
\url{https://github.com/FLC-QU-hep/getting_high}.}. 


%Early progress was made on supervised classification of 
%known particles~\cite{jet_images2,jets_w,jets_qg2,jets_top,deep_top1}
%to the point where powerful network architectures are now 
%available~\cite{jets_comparison,particlenet,jedinet,DeepJet}
%and the focus lies on improving the stability~\cite{pivot,disco,aussies,bayes,bayes2}, the experimental 
%understanding~\cite{ben_unc,ATLASTop,ATLASCorrelation,CMSTop}
%of these approaches as well as on developing new tools of statistical inference~\cite{KyleInference,INFERNO}.

Advanced machine learning methods, based on deep neural networks, are rapidly transforming and improving the way to
explore the fundamental interactions of nature in particle physics --- see for example Ref.~\cite{jets_comparison} 
for a recent overview of neural network architectures developed to identify hadronically decaying top quarks.
However, we are only beginning to explore the potential benefits from unsupervised techniques designed to  
model the underlying high-dimensional density distribution of data. This allows, e.g., anomaly detection
algorithms to identify signals from new physics theories without making  specific model assumptions~\cite{weak6,weak7,weak8,koalahunting,TaoNovelty,tagntrain,anode,SALAD,ALAD,ATLASAnomaly}.
Furthermore, once the phase space density is encoded in a neural network, it can be sampled from very efficiently. 
This makes synthetic models of particle interactions  many orders of magnitude faster than
classical approaches.


%Calorimeters are a crucial part of experiments in high energy physics, where primary particles transverse through and interact with layers made of dense material and deposit their energies.
%As a result, a shower is initiated and can be seen as a sequence of stochastic interaction of the primary and secondary particles with the detector material. These sequential interactions of particles are described by the GEANT4\cite{g4} program with great accuracy.
Calorimeters are a crucial part of experiments in high energy physics, where the incident primary particles create showers of secondary
particles in dense materials that are used to measure the energy. In sandwich calorimeters, layers of dense materials are interleaved with
sensitive layers recording energy depositions from secondary shower particles mostly from ionization. The details of the shower development via
creation of secondary particles as well as their energy loss is typically simulated with great accuracy using the GEANT4~\cite{g4} toolkit.

The crucial role of calorimeter simulation as a time-consuming bottleneck in the  simulation chain at the LHC is well established.
For example, the ATLAS experiment uses more than half of its total CPU time on the Grid for Monte Carlo simulation, which in turn is entirely
dominated by the calorimeter simulation~\cite{atlas_fastsim}. 

%For planned future experiments with higher spatial resolution, more read-out channels and
%a larger amount of simultaneous interactions, this problem is exacerbated. Furthermore,
%designs developed in the context of future colliders, are also being used to upgrade
%detectors at the LHC for upcoming data-taking periods

%These factors make the timely development of precise simulation tools for high-resolution
%detectors relevant and motivate our investigation of a prototype calorimeter for the ILD.

While generative neural network techniques promise enormous speed-ups for simulating the calorimeter response, it is
of extreme importance that all relevant physical shower properties are reproduced accurately in great detail.
This is particularly challenging for highly granular calorimeters, with a much higher spatial resolution,
foreseen for most future colliders. Such concepts, as developed for the International Linear Collider (ILC), are also being used to upgrade
detectors at the LHC for upcoming data-taking periods. One prominent example is the calorimeter endcap upgrade of the CMS experiment~\cite{hgcal_tdr} with about 6 million readout channels.
These factors make the timely development of precise simulation tools for high-resolution 
detectors relevant and motivate our investigation of a prototype calorimeter for the International Large Detector (ILD).

Outside of particle physics, generative adversarial neural networks~\cite{GAN} (GANs) have been used to produce synthetic data 
--- such as photo-realistic images~\cite{StyleGAN} --- with great success. 
An alternative to GANs for simulation are Variational Autoencoders~\cite{VAE} (VAE). 
A VAE consists of an encoder mapping from input data to a latent space, and a decoder, which maps 
from the latent space to data. 
If the probability distribution in latent space is known, it can be sampled from and
used to generate synthetic data. 
A third path towards generative models is offered by normalizing flows~\cite{NICE,RealNVP,rezende2015variational,papamakarios2019normalizing,KyleFlow}. In such models, a simple base probability distribution is transformed by a series of invertible mappings into  a complex shape. 

Recently, a novel architecture unifying several generative models such as GANs, VAEs and others
%, AAEs \cite{AAE}, InfoVAEs \cite{InfoVAE} and VAE-GANs \cite{VAE-GAN} 
was proposed: the Bounded-Information-Bottleneck auto\-en\-co\-der (BIB-AE)~\cite{BIB-AE}. We will show that by using a modified BIB-AE for generation we
can accurately model all tested relevant physics distributions. A detailed introduction to this 
architecture is provided in Section~\ref{sec:BIBAE}.

Specifically in particle physics, first results for the simulation of calorimeters focused on GANs achieved an impressive speed-up by up to five orders of magnitude compared
to GEANT4~\cite{CaloGAN2,CaloGAN,CaloGAN3}.
Similarly, an approach using a Wasserstein-GAN (WGAN) architecture achieved realistic modeling of particle showers in
air-shower detectors~\cite{ErdmannWGAN} and a sampling high granularity calorimeter~\cite{ErdmannWGAN2}.
In the context of future colliders, an architecture inspired by GANs was used 
for the fast simulation of showers in a high resolution electromagnetic calorimeter~\cite{Sofia}.
Generative models based on VAE and WGAN architectures were studied for concrete application by the ATLAS collaboration~\cite{ATLAS_Gen,ATLAS_Gen2, ATLAS_Gen3}.

Beyond producing calorimeter showers, generative models in HEP have also been 
explored for modeling
muon interactions with a dense target~\cite{SHiPGAN},
parton showers~\cite{Bothmann,Monk,JUNIPR,LundCycleGAN},
phase space integration~\cite{badger,Klimek:2018mza,Bendavid:2017zhk,Bothmann:2020ywa},
event generation~\cite{PandolfiGAN,Otten:2019hhl,KaustuvGAN,DiJetGAN,LHCGAN,FlowGeneration},
event subtraction~\cite{ButterSubtraction} and unfolding~\cite{GANFolding}.

The rest of this paper is organised as follows: in Section~\ref{data} we introduce the concrete
problem and training data, in Section~\ref{models} the used generative architectures are discussed,
and in Section~\ref{results} the obtained results are presented and compared. Finally, Section~\ref{closing}
provides conclusions and outlook.

%An early problem was the correct classification of collimated showers of hadrons --- so-called jets --- to the particle that initiated them. 
%This includes the correct identification of top-quarks, W-bosons, bottom-quarks, gluons, and long-lived particles. \textbf{GK: Cite the key papers}. 
%Interesting open problems --- such as understanding uncertainties, stability, and interpretability  --- still exist, but the basic problem of
%supervised classification is essentially solved. 

%Alas, much more can be achieved by unsupervised approaches that learn to model the underlying high-dimensional density distribution of data. 
%This allows the construction of novelty detectors which are able to potentially identify signals from new physical theories without an 
%explicit model bias. On the other hand, density distributions encoded in a network can usually be sampled from much faster than the underlying (slow) 
%model, enabling fast generative models. The main target for these generative models in particle physics, is the fast simulation of calorimeters.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% DATA SET
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Data Set}
\label{data}

\begin{figure}[b]
    \centering
    \includegraphics[width=0.42\textwidth]{./figures/ild_photon_shower_60GeV-3_white_bg_noEcal}
    \caption{A simulated 60 GeV photon shower in the ILD detector, as used in the training data. Here a coordinate system different from the original ILD detector is chosen, where the z-axis is parallel to the photon momentum and the shower development. }
    \label{fig:ecal}
\end{figure}


The ILD~\cite{ILD-IDR} detector is one of two detector concepts proposed for the ILC. It is optimized for
Particle Flow (PFA), an algorithm that aims at reconstructing every individual particle in order to optimize the overall detector resolution. ILD combines high-precision tracking and vertexing capabilities with very good hermiticity and highly granular
electromagnetic and hadronic calorimeters. For this study, one of the two proposed electromagnetic calorimeters for ILD, the Si-W ECal is chosen.
It consists of 30  active silicon layers in a tungsten absorber stack with 20 layers of $2.1~\textrm{mm}$ followed by 10 layers of  $4.2~\textrm{mm}$
thickness respectively. The silicon sensors have $5\times 5~\textrm{mm}^2$ cell sizes. 
Throughout this work, we project the sensors onto a rectangular grid of  $30\times30\times30$~cells. Each cell
in this grid corresponds to exactly one sensor. As the underlying geometry of sensors in a
realistic calorimeter prototype is not exactly regular, we will encounter some effects of this staggering. 
This makes the learning task more challenging for the network, but does not pose a fundamental problem.
Architectures that more accurately encode irregular calorimeter geometries in neural networks exist~\cite{CaloGraphs}, but are not the focus of this work.


\begin{figure}[b]
    \centering
    %\includegraphics[width=0.31\textwidth]{./figures/Shower_Real_50_GeV_CollapseZ.png}
    %\includegraphics[width=0.31\textwidth]{./figures/Shower_Real_50_GeV_CollapseX.png}
    %\includegraphics[width=0.31\textwidth]{./figures/Shower_Real_50_GeV_CollapseY.png}
    %\includegraphics[width=0.31\textwidth]{./figures/Shower_Real_50_GeV_CollapseZSum.png}
    %\includegraphics[width=0.31\textwidth]{./figures/Shower_Real_50_GeV__CollapseXSum.png}
    \includegraphics[width=0.35\textwidth]{./figures/Shower_Real_50_GeV_CollapseYSum.png}
    \caption{
    %Projections of a 50 GeV GEANT4 photon shower along the z, x and y direction (top) and overlays of 2000 such projections (bottom)
    Overlay of 2000 projections of a 50~GeV GEANT4 photon shower along the y direction.}
    \label{fig:showers_projection}
\end{figure}


ILD uses the iLCSoft~\cite{ilcsoft} ecosystem for detector simulation,
reconstruction and analysis. For the full simulation with GEANT4, a detailed and realistic detector model implemented in DD4hep~\cite{dd4hep} is used.
The training data of photon showers in the ILD ECal are simulated with GEANT4 version 10.4 (with \textrm{QGSP\_\,BERT} physics list) and DD4hep version 1.11.
The photons are shot at perpendicular incident angle into the ECal barrel with energies approximately uniformly distribu\-ted between 10-100 GeV. All incident photons are aimed at the $x-y$ center of the grid --- i.e. at
the point in the middle between the four most central cells of the front layer.
An example event display showing such a photon shower is depicted in Figure~\ref{fig:ecal}. 
%


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.4\textwidth]{./figures/GEANT4_Full_incident_E.png}
%    \caption{Energy spectrum of the training sample.}
%    \label{fig:spectrum}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.35\textwidth]{./figures/Shower_Real_50_GeV3d.png}
%    \caption{Example of a 50 GeV photon shower in 3D. 
%    The color of each grid cell encodes the energy measured by the corresponding sensor.
%    }
%    \label{fig:showers}
%\end{figure}


%The energy distribution of the photons used for training is shown in Figure~\ref{fig:spectrum}.
%A slight slope is visible in the distribution. It is an artefact of the generation setup 
%caused by the specific scripts used for generating the photons 
%and no effect on the network performance is expected. 

The incoming photon enters from the bottom at $z=0$ and traverses along the z-axis, hitting cells in the center of the $x-y$ plane.
No variations of the incident angle and impact point are performed in this study. 
The overlay of 2000 showers summed over the y-axis
%The projection of an example shower onto the three axes are shown in
is shown in Figure~\ref{fig:showers_projection}. As can be seen, %from the projection onto the y-axis,
the cells in the ILD ECal are staggered due to the specific barrel geometry.
The whole data set for training consists of 950k showers with continuous energies between 10-100 GeV. 
For the evaluations we generated additional, statistically independent, sets of events: 40k events uniformly distributed between 10-100 GeV and 
4k events each at discrete energies in steps of 10~GeV between 20 and 90~GeV.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% GENERATIVE MODELS
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Generative Models}

\label{models}

Generative models are designed to learn an underlying data distribution in a way that
allows later sampling and thereby producing new examples. In the following, we first
present two approaches --- GAN and WGAN --- which 
represent the state-of-the-art in generating calorimeter data and which we use to benchmark our
results. We then introduce BIB-AE as a novel approach to this problem and discuss further 
refinement methods to improve the quality of generated data.

% Generative models aim to learn any kind of data distribution using unsupervised learning, where labels for the data do not exist. The primary goal is to learn a distribution which is as close as possible to the true data distribution. Two of the most popular approaches are Variational Autoencoders (VAE) and Generative Adversarial Networks (GAN). While VAE tries to learn a low-dimensional latent representation of the training data, GAN aims to approximate probability distribution function that the training data is assumed to be drawn from.

%Essentially, a GAN consists of two functions: a generator 
%producing synthetic data examples from random noise, and a discriminator, distinguishing data 
%produced by the generator from real examples. These functions are implemented as neural networks
%and the weights are optimised to solve the min-max problem of competing generator and discriminator. 
%This basic template can be modified in a number of ways e.g. to allow conditioning~\cite{Conditional};
%or to improve the training stability via alternative definitions of the optimisation target (loss function)
%as in the Wasserstein-GAN~\cite{WGAN,WGAN2} (WGAN) approach.

%As traditional VAEs do not rely on an adversarial term in the loss function, 
%they are easier to train compared to GANs but also produce less realistic examples, i.e. generating more blurry images \cite{VAE-GAN}. \done{TODO: Can someone track down a credible citation for this?}

\subsection{Generative Adversarial Network}

\label{sec:GAN}


The GAN architecture was proposed in 2014~\cite{GAN} and had remarkable success
in a number of generative tasks. It introduces generative models by an adversarial process, in which a generator $G$ competes against an adversary (or discriminator) $D$. The goal of this framework is to train $G$ in order to generate samples $\widetilde{x}=G(z)$ out of noise $z$, which are indistinguishable from real samples $x$. The adversary network $D$ is trained to maximize the probability of correctly classifying whether or not a sample came from real data
using the binary cross-entropy.
The generator, on the other hand, is trained to fool the adversary $D$.
This is represented by the loss function as 
\begin{equation}
\label{eqn:JS}
\begin{split}
%    \min_G \max_D \mathbb{E}_{x\sim p_{data(x)}}[ & \log D(x)] \\
%    & + \mathbb{E}_{z\sim p_z(z)}[\log (1-D(G(z)))],
    L = \min_G \max_D \mathbb{E}[ & \log D(x)] + \mathbb{E}[\log (1-D(G(z)))],
\end{split}
\end{equation}
and a schematic of the GAN training is provided in Fig.~\ref{fig:VGAN}~(top). 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{./figures/VGAN.png}
    
    \vspace{0.3cm}
    
    \includegraphics[width=0.48\textwidth]{./figures/WGAN.png}
    \caption{Overview of the GAN (top) and WGAN (bottom) architectures.
    The blue line shows where the true energy is used as an input. 
    The loss functions and feedback loops are explained in the text. 
    }
    \label{fig:VGAN}
\end{figure}

%\begin{figure}[t]
%    \centering
%    
%    \caption{Overview of the Wasserstein-GAN architecture.}
%    \label{fig:WGAN}
%\end{figure}


For practical applications, the GAN needs to simulate showers of a specific energy. To this end, 
we parameterise generator and discriminator as functions of the photon energy $E$~\cite{Parametrised}.



The original formulation of a GAN produces a generator that
minimizes the Jensen-Shannon divergence between true and generated data.
In general, the training of GANs is known to be technically challenging and subject to
instabilities~\cite{WGAN2}. Recent progress on generative models 
improves upon this by modifying the learning objective.

%Recent progress in the GAN field focus on improving the stability and quality of the vanilla GAN training by using different approaches for discriminator. 

%, where $D$ is a binary classifier that minimizes the  distribution and one assumed in generator, training process is very difficult and subject to instabilities. Recent progress in the GAN field focus on improving the stability and quality of the vanilla GAN training by using different approaches for discriminator. 

\subsection{Wasserstein-GAN}

\label{sec:WGAN}



One alternative to classical GAN training is to use the Wasserstein-1 distance, also known as earth mover's distance, as a loss function. This distance evaluates dissimilarity between two multi-dimensional distributions and informally gives the cost expectation for moving a mass of probability along optimal transportation paths~\cite{optimal_transport}.  Using the Kantorovich-Rubinstein duality, the Wasserstein loss can be calculated as
\begin{equation}
    \label{eqn:wloss}
    L = \textrm{sup}_{f\in \textrm{Lip}_1}\{\mathbb{E}[f(x)] - \mathbb{E}[f(\tilde{x})]\}.
\end{equation}
The supremum is over all 1-Lipschitz functions $f$, which are approximated by a discriminator network $D$ during the adversarial training. This discriminator is called \textit{critic} since it is trained to estimate the Wasserstein distance between real and generated images.
%; instead of a binary classification (i.e fake or generated) as its GAN counterpart does. 

%In addition, it has been reported that the loss function in (\ref{eqn:wloss}) appears to be correlated with sample quality~\cite{WGAN}, which is not the case for a vanilla GAN.

In order to enforce the 1-Lipschitz constraint on the critic~\cite{WGAN2}, a gradient penalty term
can be added to (\ref{eqn:wloss}), yielding the critic loss function:
\begin{equation}
    \label{eqn:wgan_gp}
    \begin{split}
    L_{\textrm{Critic}} = \mathbb{E}[D(G(z))] & - \mathbb{E}[D(x)]  \\
    & + \lambda\,\, \mathbb{E}[(\parallel\nabla_{\hat{x}}D(\hat{x})\parallel_2 - 1)^2 ],
    \end{split}
\end{equation}
where $\lambda$ is a hyper parameter for scaling the gradient penalty. The term $\hat{x}$ is a mixture of real data $x$ and generated $G(z)$ showers. Following~\cite{WGAN2}, it is sampled uniformly along linear interpolations between $x$ and $G(z)$. %motivated by the fact that the optimal critic has straight lines with gradient norm 1 connecting coupled points from the underlying probability distribution of $x$ and $G(z)$\cite{WGAN2}.

Finally, we again need to ensure that generated showers accurately resemble photons of the 
requested energy. We achieve this by parametrising the generator and critic networks in $E$ and
by adding a constrainer~\cite{ErdmannWGAN2} network $a$.
The loss function for the generator then reads:
\begin{equation}
    \label{eqn:constrE}
    \begin{split}
    L_{\textrm{Generator}} = & -\mathbb{E}[D(\tilde{x},E)] \\
    & + \kappa\cdot \mathbb{E}[\left| (a(\tilde{x}) - E)^2 - (a(x) - E)^2 \right| ],
    \end{split}
\end{equation}
where $\tilde{x}$ are generated showers and $\kappa$ is the relative strength of the conditioning term. 
This combined network is illustrated in Fig.~\ref{fig:VGAN}.
The constrainer network is trained solely on the GEANT4 showers; its weights are fixed during the generator training.  We use the mean absolute error as loss: 
\begin{equation}
    \label{eqn:constrE_sup}
    L_\textrm{Constrainer} = \left|E - a(x)\right|.
\end{equation}


%Following the formalism of , we would like to have our generated showers which must be associated with initial state of incident particle's kinematics, achieved by explicitly modifying the generator's dependency in our setup: $G(z,E)$, where $E$ is the energy of incident photons. This is referred as \textit{conditioning} and is accomplished with the help of another neural network, network $a_{\theta}$, parametrized by weights $\theta$. It evaluates how well the generated samples contain the characteristics of incident photon energy. This is done by introducing an extra term in the generator's loss function:
%\begin{equation}
%    \label{eqn:constrE}
%    L_{generator} = -\mathbb{E}[D(\tilde{x},E)] + \kappa\cdot \mathbb{E}[\left| \{a_{\theta}(\tilde{x}) - E\}^2 - %\{a_{\theta}(x) - E\}^2 \right| ],
%\end{equation}
%where $\tilde{x}$ is generated showers; $\kappa$ is a hyperparameter for the conditioning term. In contrast to \cite{ErdmannWGAN2}, we train $a_{\theta}$ network with mean absolute error: 
%\begin{equation}
%    \label{eqn:constrE_sup}
%    L = \left|E - a_{\theta}(x)\right|.
%\end{equation}

\subsection{Bounded Information Bottleneck-Autoencoder}

\label{sec:BIBAE}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{./figures/BAE_PP.png}
    \caption{Diagram of the BIB-AE architecture, including the additional MMD term defined in Sec.~\ref{sec:MMD}
    and the Post Processor Network defined in Sec.~\ref{sec:PP}. The blue line shows where the true energy is used as an input. 
    The loss functions and feedback loops are explained in the text. }
    \label{fig:BAE_PP}
\end{figure*}

Autoencoder architectures map input to output data via a latent space. 
Using a structured latent space allows later sampling and thereby generating new data.
The BIB-AE~\cite{BIB-AE} architecture was introduced as a theoretical overarching generative model.
Most commonly employed generative models --- e.g. GAN \cite{GAN}, VAE \cite{VAE}, and adversarial autoencoder (AAE)~\cite{AAE} --- can be seen as different subsets of the BIB-AE.
This leads to better control over the latent space distributions and promises better generative performance and interpretability. 
In the following, we focus on the practical advantage gained from utilizing these the components and refer to the original publication~\cite{BIB-AE} for a
information-theoretical discussion.

As it is an overarching model, an instructive way for describing the base BIB-AE framework is by taking a VAE and expanding upon it. A default VAE consist of four general components: an encoder, a decoder, a latent-space regularized by the Kullback--Leibler divergence (KLD), and an $L_N$-norm to determine the difference between the original and the reconstructed data. These components
are all present as well in the BIB-AE setup.
Additionally, one introduces a GAN-like adversarial network, trained to distinguish between real and reconstructed data, as well as a sampling based method of regularizing the latent space, such as another adversarial network or a maximum mean discrepancy (MMD, as described in the next section) term. In total this adds up to four loss terms: The KLD on the latent space, the sampling regularization on the latent space, the $L_N$-norm on the reconstructed samples and the adversary on the reconstructed samples. The guiding principle behind this is that the two latent space and the two reconstruction losses complement each other and, in combination, allow the network to learn a more detailed description of the data.

Our specific implementation of the BIB-AE framework is shown in Fig.~\ref{fig:BAE_PP}. For our sampling based latent regularization we use both an adversary and an MMD term. The adversaries are implemented as critics trained with gradient penalty, similar to the WGAN approach. The main difference in our setup is that we replaced the $L_N$-norm with a third critic trained to minimize the difference between input and reconstruction. We chose this because we found that using the $L_N$-norm to compare the input and the reconstructed output resulted in smeared out images.
%~\footnote{A detailed description of MMDs can be found in the next section}. 

For the precise implementation the loss functions we define the encoder network $E$, the decoder network $D$, the latent critic $C_L$, the critic network $C$, 
and the difference critic $C_D$. % and the sample for the data set $x$. 
The loss function for the latent critic $C_L$ is given by
\begin{equation}
    \label{eqn:bibae_crit_L}
    \begin{split}
    L_{C_{L}} = \mathbb{E}[C_L(E(x))] & - \mathbb{E}[C_L(\mathcal{N}(0,1))]  \\
    & + \lambda\,\, \mathbb{E}[(\parallel\nabla_{\hat{x}}C_L(\hat{x})\parallel_2 - 1)^2 ].
    \end{split}
\end{equation}
Here $\hat{x}$ is a mixture of the encoded input image $E(x)$ and samples from a normal distribution $\mathcal{N}(0,1))$.
The loss function for the main critic $C$ is given by
\begin{equation}
    \label{eqn:bibae_crit}
    \begin{split}
    L_{C} = \mathbb{E}[C(D(E(x)))] & - \mathbb{E}[C(x)]  \\
    & + \lambda\,\, \mathbb{E}[(\parallel\nabla_{\hat{x}}C(\hat{x})\parallel_2 - 1)^2 ].
    \end{split}
\end{equation}
Where $\hat{x}$ is a mixture of the reconstructed image $D(E(x))$ and the original images $x$.
Finally, the loss function for the difference critic $C_D$ is given by
\begin{equation}
    \label{eqn:bibae_crit_D}
    \begin{split}
    L_{C_D} = \mathbb{E} & [C_D(D(E(x)) - x)]  - \mathbb{E}[C_D(x - x=0)]  \\
    & + \lambda\,\, \mathbb{E}[(\parallel\nabla_{\hat{x}}C_D(\hat{x})\parallel_2 - 1)^2 ].
    \end{split}
\end{equation}
Where $\hat{x}$ is a mixture of the difference $D(E(x)) - x$ and the difference $x - x=0$.
  
With different $\beta$ factors 
giving the relative weights for the individual loss terms,
the combined loss for the encoder and decoder parts of the BIB-AE can be expressed as:
\begin{equation}
    \label{eqn:BIBAE}
    \begin{split}
    L_{\textrm{BIB-AE}} = & - \beta_{C_L} \cdot \mathbb{E}[C_L(E(x))] \\
    & - \beta_{C} \cdot \mathbb{E}[C(D(E(x)))] \\
    & - \beta_{C_D} \cdot \mathbb{E}[C_D(D(E(x)) - x)] \\
    & + \beta_{\textrm{KLD}} \cdot \textrm{KLD}(E(x)) \\
    & + \beta_{\textrm{MMD}} \cdot \textrm{MMD}(E(x),\mathcal{N}(0,1))).
    \end{split}
\end{equation}


%We noticed, however, that the $L_N$-norm was incapable of capturing the sharp features in our shower images. This caused the resulting images to be overly smooth. This effect was most pronounced in the outer regions of the shower, where the $L_N$-norm VAE could not reproduce the sparse structure surrounding the shower core. The first set was therefore to replace the $L_N$-norm with a critic network, similar to the one used in the Wasserstein GAN. This resulted in sharp images with the desired outer structures. The critic network only incentives the decoder to produce realistic looking showers, not to reconstruct the input image, making this approach equivalent to a GAN. Based on our findings this made it difficult for the network to learn global distribution such as the shape of the peak in deposited energy spectrum. We decided to remedy this problem by reintroducing a term that incentives reconstructing the original images. Since combinations of the Critic network with a $L_N$-norm suffered from the same problems as a standalone $L_N$-norm, we use a second Critic which takes the pixel-wise difference between the original and reconstructed images as its input and tries to minimize these. In the actual implementation both these Critics are combined into one network, as this allows the network to learn the ideal weighting of the standard Critic and difference Critic contribution. 

%The final loss term in this setup is an adversarial Critic that compares the sampled latent space to an equal amount of samples drawn form normal distributions, similar to the latent Critic in an AAE. In a standard VAE there is an equilibrium between the KLD- and the reconstruction loss term, since the KLD is trying to minimize the amount of information in the latent space and the reconstruction loss is trying to maximize the encoded information. This means the VAE has a sort of information budget, describing how much information it can encode in its latent space. For a generative model the ideal usage of this budget would be to have every latent space distribution differ slightly form a normal distribution, as this means they can still be approximated reasonably well by a normal distribution during the generation process. In practice it is, however, more common to have most of the latent distributions be perfect normal distributions, while a small number differs greatly form a normal distribution (Can we cite jack here somehow??). This is problematic since these few distributions carry most of the relevant information, but are also hard to sample during generation. This is the reason we employ the latent space Critic. It will discourage these individual, deviating distributions and thereby force the network the spread the information evenly throughout the latent space. 
%
%
%

\subsection{Maximum Mean Discrepancy}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.22\textwidth]{./figures/Shower_Real_50_GeV3d.png}
    \hspace{0.06\textwidth}
    \includegraphics[width=0.22\textwidth]{./figures/Shower_3D_paper_GAN_50_GeV3d.png}
    \includegraphics[width=0.22\textwidth]{./figures/Shower_3D_paper_WGAN_50_GeV3d.png}
    \includegraphics[width=0.22\textwidth]{./figures/Shower_3D_paper_BiBAE_PP_50_GeV3d.png}
    \caption{
    Examples of individual 50~GeV photon showers generated by GEANT4 (left), the GAN (center left), WGAN (center right), and BIB-AE (right)
    architectures. Colors encode the deposited energy per cell.}
    \label{fig:results_3dplots}
\end{figure*}

\label{sec:MMD}

One major challenge in generating realistic photon showers is the spectrum of the individual cell energies, which is shown in  Fig.~\ref{fig:results_diffdist1}~(left)
in Section~\ref{results}.
The real spectrum shows an edge around the energy that a minimal ionizing particle (MIP) would deposit. Since the well-defined energy deposition of a MIP is often used to calibrate a calorimeter, we cannot simply ignore it. However, we found that purely adversarial based methods tend to smooth out this feature, an observation in line with other efforts to use generative networks for shower simulation~\cite{ErdmannWGAN2}. A way of dealing with this is using MMD~\cite{MMD_base} to compare and minimize the distance between the real $(D_{R})$ and fake $(D_{F})$ hit-energy distributions:
\begin{align}
\label{eq:mmd}
\begin{split}
    \textrm{MMD}(D_{R}, D_{F}) = & \langle k(x,x') \rangle + \langle k(y,y') \rangle  \\
    & - 2\langle k(x,y) \rangle ,
\end{split}
\end{align}
where $x$ and $y$ are samples drawn from $D_{R}$ and $D_{F}$ respectively and $k$ is any positive definite kernel function. MMD based losses have previously been used in the generation of LHC events~\cite{LHCGAN}. 

A naive implementation of the MMD would be to compare every pixel value from a real shower with every value from a generated shower. This approach is however not feasible since it would involve computing Equation (\ref{eq:mmd}) approximately $(30^{3})^{2}$ times for each shower.
To make the MMD calculation tractable, we introduce a novel version of the MMD, termed Sorted-Kernel-MMD. We first sort both, real and generated, hit-energies in descending order, and then  take the $n$ highest fake energies and compare them to the $n$ highest real energies. Following this we move the $n$-sized comparison window by $k$ and recompute the MMD. This process is repeated $\frac{N}{k}$-times, where $N$ is the total number of pixels one wants to compare. The advantage of this approach is two-fold, for one the number of computations is linear in $N$, 
%as opposed to the others \fix{KK: which others?}, 
as opposed to the naive implementation
which shows quadratic behavior. 
The second advantage is that energies will only be compared to similar values, thereby incentivising the model to fine-tune 
the energy. 
%\fix{KK: I don't understand the sentence}.  
Specifically, the values  N=2000, k=25, and n=100 are used. 
%The problem can be alleviated by ignoring most of the empty pixels. From the top right plot in fig.~\ref{fig:results_diffdist} we can see that the maximum amount of non-zero pixels is approximately~$2000$ of the total~$2700$. Therefore we can apply the MMD only to the $2000$ highest value pixels in each image. This allows us to cut down the number of evaluations to $2000^2$. 
%This, however still proved as to computationally expensive to be useful. 
In our experiments, adding this MMD term with the kernel function 
\begin{equation}
    k(x,x^{\prime}) = e^{- \alpha (x^{2} + x^{\prime 2} - 2 x x^{\prime})} 
\end{equation} 
with $\alpha = 200$ to the loss term of either a GAN or a BIB-AE fixes the per-cell hit energy spectrum to be near identical to the training data. This however comes at a price, as the additional pixels with the energies used to fix the spectrum are often placed in unphysical locations, specifically at the edges of the $30 \times 30 \times 30$ cube. %This is because these areas are sparsely populated in the training data, which seems to cause the critic networks to view them as less important. Therefore placing the additional hits there is an easy way for the network to minimize the MMD term.


\subsection{Post Processing}

\label{sec:PP}

In the previous section we found that using an MMD term in the loss function represents a trade off between correctly reproducing either the hit energy spectrum or the shower shape. 
To solve this, we split the problem into two networks that are applied consecutively but trained with different loss functions. The first network is a GAN or BIB-AE trained without the MMD term. This produces showers with correct shapes, but an incorrect hit-energy spectrum. The second network then takes this shower as its input and applies a series of convolutions with kernel size one. Therefore this second network can only modify the values of existing pixels, but not easily add or remove pixels. This second network, here called Post Processor Network, is trained using only the MMD term to fix the hit energy spectrum, and the mean squared error (MSE) between the input and output images, ensuring the change from the Post Processor Network is as minimal as possible. 



%With this setup we are then able to produce showers with both the correct shape and energy spectrum.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% RESULTS
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Results}



\label{results}

In the following we present the ability of our generative models to accurately predict a number
of per-shower variables as well as global observables and analyse the achievable gain in computing performance. 
We include our implementation of a simple GAN~(Sec.~\ref{sec:GAN}), 
a WGAN with additional energy constrainer (Sec.~\ref{sec:WGAN}),
and a BIB-AE with energy-MMD and post processing (Secs.~\ref{sec:BIBAE},~\ref{sec:MMD} and ~\ref{sec:PP}).
A detailed discussion of the architectures and training hyper parameters can be found in Appendix~\ref{hyper}.
All architectures are trained on the same sample of 950k GEANT4 showers.
Tests are either shown
for the full momentum range (labeled \textit{full spectrum}) or for specific shower energies (labeled 
with the incident photon energy in GeV).

\subsection{Physics Performance}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{./figures/3D_paper_Uncut_hit_E_dist.png}
    \includegraphics[width=0.42\textwidth]{./figures/3D_paper_occ_dist_3ofaKind.png}
    \caption{Differential distributions comparing the per-cell energy (left) and the number of hits (right) between GEANT4 and the different generative models.
    Shown are GEANT4 (grey, filled), our GAN setup (blue, dashed), our WGAN (red, dotted) and the BIB-AE (green, solid).
    The energy per-cell is measured in MeV for the bottom axis and in multiples of the expected energy deposit of a minimum ionizing particle (MIP) for
    the top axis.
    }
    \label{fig:results_diffdist1}
\end{figure*}






We first verify in Fig.~\ref{fig:results_3dplots} that the showers generated by
all network architectures visually appear to be acceptable compared to GEANT4.
Were we attempting to generate \textit{cute cat pictures}, our work would be done already at this point. 
Alas, these shower images are eventually to be used as realistic substitutes in physics analyses so we 
need to pay careful attention to relevant differential distributions and correlations.



\begin{figure*}[h]
    \centering
    %\includegraphics[width=0.31\textwidth]{./figures/3D_paper_Uncut_hit_E_dist.png}
    \includegraphics[width=0.3\textwidth]{./figures/3D_paper_single_E_dist_3ofaKind.png}
    %\includegraphics[width=0.31\textwidth]{./figures/3D_paper_occ_dist_3ofaKind.png}
    \includegraphics[width=0.3\textwidth]{./figures/3D_paper_CenterOfGravity_dist.png}\\
    \includegraphics[width=0.3\textwidth]{./figures/3D_paper_spinal_E_dist.png}
    \includegraphics[width=0.3\textwidth]{./figures/3D_paper_radial_E_dist.png}
    \caption{Additional differential distributions comparing physical observables between GEANT4 and the different generative models.
    Shown are GEANT4 (grey, filled), our GAN setup (blue, dashed), our WGAN (red, dotted) and the BIB-AE (green, solid).
    }
    \label{fig:results_diffdist2}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.34\textwidth]{./figures/3D_paper_Calo_Mean_relative.png}
    \includegraphics[width=0.34\textwidth]{./figures/3D_paper_Calo_Width_relative.png}
    \caption{Distribution of mean ($\mu_{90}$, left) and relative width ($\sigma_{90}/\mu_{90}$, right)  of the energy deposited in the calorimeter for various incident particle energies.
    In the bottom panels, the relative offset of these quantities with respect to the GEANT4 simulation is shown.}
    \label{fig:results_mean}
\end{figure*}



In Figure~\ref{fig:results_diffdist1} a comparison between two differential distributions for 
all studied architectures and GEANT4 is shown. The left plot compares the per-cell hit-energy spectrum
averaged over showers for the full spectrum of photon energies. 
We observe that while the high-energy hits are well described by all generative models, both GAN and WGAN fail to capture the bump around 
$0.2$~MeV. The BIB-AE is able to replicate this feature thanks to the Post Processor Network.\footnote{We studied applying post processing to the WGAN architecture as well. This is discussed in Appendix~\ref{A:WGAN_PP}.} This energy corresponds to the most probable energy loss of a MIP passing a silicon sensor of the ILD Si-W ECal at perpendicular incident angle. Since this is a well-defined energy, it can be used in highly granular calorimeters for the equalisation of the cell response as well as for setting an absolute energy scale. 
It also leads to a sharp rise in the spectrum, as lower energies can only be deposited by ionizing particles that pass only a fraction of the thickness at the edges of sensitive cells or that are stopped.
The region below half a MIP, corresponding to around 0.1~MeV,  is shaded in dark grey. These cell energies are very small and therefore 
will be discarded in a realistic calorimeter. For the following discussion cell energies below 0.1~MeV will therefore not be considered and only cells above this cut-off are included in all other performance plots and distributions.

Next, the plot on the right shows the number of hits for three discrete photon energies (20 GeV, 50 GeV, and 80 GeV). 
Here, the GAN and WGAN setups slightly underestimate the total number of hits, while the BIB-AE accurately models the mean and width 
of the distribution. This behavior can be traced back to the left plot. Since we apply a cutoff removing hits below $0.1\ \textrm{MeV}$, a model that does not correctly reproduce the hit-energy spectrum around the cut-off will have difficulties correctly describing the number of hits. 

Additional distributions are shown in Fig.~\ref{fig:results_diffdist2}. The top left depicts the visible energy distribution for the same three discrete photon energies. 
Both, the shape, center and width of the peak are well reproduced for all models. 
Due to the sampling nature of the calorimeter under study, the visible energy is of course much lower
than the incoming photons' energy.
    
In the top right and bottom two plots we compare the spatial properties of the generated showers. 
First, on the top right, the position of the center of gravity along the z axis
is shown. The GEANT4 distribution is well modelled by the GANs, however there are slight deviations for the BIB-AE.
A detailed investigation of this discrepancy showed that the z axis center of gravity is largely encoded in a single
latent space variable. A mismatch between the observed latent distribution for real samples and the normal distribution 
drawn from when generating new samples directly translates into the observed difference. Sampling from a modified
distribution would remove the problem. 

Finally, the two plots on the bottom show the longitudinal and radial energy distributions.
We see that while all models are able the reproduce the bulk of the distributions very well, deviations for the WGAN appear around the edges. 

%This is connected to how the BIB-AE encodes the center of gravity in its latent space [Not sure how much to add here, this seems like it belongs into the latent space follow up]. 


We next test how well the relation of visible energy to the incident photon energy is reproduced. To this end we use a GEANT4 sample where we simulated photons at discrete energies ranging from 20 to 90 GeV in 10 GeV steps. We then use our models to generate showers for these energies and calculate the 
mean and root-mean-square of the $90\%$~core of the distribution, labeled $\mu_{90}$ and $\sigma_{90}$ respectively, 
for all sets of showers. The results are shown in Fig.~\ref{fig:results_mean}. Overall the mean (left) is correctly modelled, showing only deviations in the order of one to two percent. 
The relative width, $\sigma_{90}/\mu_{90}$ (right) looks worse: GAN and WGAN overestimate the GEANT4 value at all energies.
%while the GAN strongly overestimates at low energies but accurately predicts the width otherwise.
While the BIB-AE on average correctly models the width, it still shows deviations of up to ten percent
at high energies. Note that the width cannot be interpreted as energy resolution of the calorimeter due to the two different absorber thicknesses used in the ECal, requiring different calibrations.
%the quantity used here is not the calorimeter energy resolution.


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{./figures/_GEANT4_correlations.png}
    \includegraphics[width=0.45\textwidth]{./figures/3D_paper_GAN_correlations_diff.png}    
    \includegraphics[width=0.45\textwidth]{./figures/3D_paper_WGAN_correlations_diff.png}
    \includegraphics[width=0.45\textwidth]{./figures/3D_paper_BiBAE_PP_correlations_diff.png}
    \caption{Linear correlation coefficients between various quantities described in the text in GEANT4 (top left). 
    Difference between these correlations in GEANT4 and GAN (top right),
    GEANT4 and WGAN (bottom left), and GEANT4 and BIB-AE with post processing (bottom right).
    %\fix{Can the axis labels be a bit bigger and the plot title be much bigger?} \fix{KK: I think this needs to be bigger in general, I can barely read the numbers in the plot}
    }
    \label{fig:results_correlations}
\end{figure*}

Finally, we verify whether correlations between individual shower properties present in GEANT4 are correctly reproduced by our generative setups. 
The properties chosen for this are: The first and second moments in x, y and z direction, labeled as $m_{1,x}$ through $m_{2,z}$, the visible energy deposited in the calorimeter $E_{\textrm{vis}}$, the energy of the simulated incident particle $E_{\textrm{inc}}$, the number of hits $n_{\textrm{hit}}$, and the ratio between the energy deposited in the 1st/2nd/3rd third of the calorimeter and the total visible energy, labeled $E_{1}/E_{\textrm{vis}}$ through $E_{3}/E_{\textrm{vis}}$. The results are shown in Fig.~\ref{fig:results_correlations}. 
The top left plot shows the correlations for GEANT4 showers. 
We then present the difference to GEANT4 for the GAN (top right), WGAN (bottom left),
and BIB-AE (bottom right). The smallest differences are observed for the GAN (absolute maximum difference of $0.2$), followed BIB-AE ($0.36$) and WGAN ($0.57$).

%Large differences of up to $0.98$ compared to GEANT4 are observed
%for the GAN. On the other hand, WGAN and BIB-AE are able to reproduce GEANT4 correlations similarly %well, with a difference of $0.41$ at most.



\subsection{Computational Performance}

Beyond  the physics performance of our generative models, discussed in the previous section, the major argument
for these approaches is of course the potential gain in production time. To this end, we benchmark the per-shower generation time both on CPU and GPU hardware architectures. In Table~\ref{table:bench}, we provide the performance for 4 (3) batch sizes for the WGAN\footnote{The time evaluation of the GAN network is not reported since the generator architecture is very similar to the WGAN.} (BIB-AE).
We observe a speed-up by evaluating generative models on GPU vs. GEANT4 on CPU of up to almost a factor of three thousand, even
for the more complex BIB-AE architecture.
Moreover, the evaluation time of our generative models is independent of the incident photon energy while this is not the case for the GEANT4 simulation.
%and expect to see faster generation by taking advantage of batch processing. 

%TODO: Understand! Except for the WGAN on GPU, higher batch sizes give faster execution times. The reason for a significant slow execution time for the WGAN at a batch size of 10 is still under investigation.  


\begin{table*}
\centering
\label{table:bench}
\caption{Overview of computational performance of WGAN and BIB-AE model, compared to GEANT4 full simulation.  Evaluated on both Intel\textsuperscript{\tiny\textregistered} Xeon\textsuperscript{\tiny\textregistered} CPU E5-2640 v4 (CPU) and NVIDIA\textsuperscript{\tiny\textregistered} V100 with 32~GB of memory (GPU). Numerical values
represent the mean and standard deviation of 25 runs.}
 \begin{tabular}{||c c l | l c| l c||} 
 \hline
 Simulator & Hardware & Batch Size& 15 GeV & Speed-up & 10-100 GeV Flat & Speed-up \\ [0.5ex] 
 \hline
GEANT4     & CPU      & N/A       &  $1445.05\pm{19.34}$ ms          & -                   & $4081.53\pm{169.92}$ ms & - \\
\hline
WGAN & CPU       & 1            &  $64.34\pm{0.58}$ ms   & \textbf{x23}           &   $63.14\pm{0.34}$ ms & \textbf{x65}\\
 &        & 10           &  $59.53\pm{0.45}$ ms  & \textbf{x24}            &   $56.65\pm{0.33}$ ms  &\textbf{x72}\\
 &        & 100          &  $58.31\pm{0.93}$ ms  & \textbf{x25}           &  $58.11\pm{0.13}$ ms &\textbf{x70}\\
 &        & 1000         &  $57.99\pm{0.97}$ ms  & \textbf{x25}           &  $57.99\pm{0.18}$ ms &  \textbf{x70}\\
\hline
BIB-AE & CPU  & 1              & $426.60\pm{3.27}$ ms & \textbf{x3}      &  $426.32\pm{3.62}$ ms & \textbf{x10} \\
 &   & 10              & $422.60\pm{0.26}$ ms & \textbf{x3}      &  $424.71\pm{3.53}$ ms & \textbf{x10}\\
 &   & 100              & $419.64\pm{0.07}$ ms & \textbf{x3}      &  $418.04\pm{0.20}$ ms  & \textbf{x10} \\
\hline
WGAN & GPU       & 1              &  $3.24\pm{0.01}$ ms     &  \textbf{x446}   & $3.25\pm{0.01}$ ms  &  \textbf{x1256}      \\
% &       & 5              &  $2.05\pm{0.01}$ ms     &  \textbf{x705}   & $2.05\pm{0.01}$ ms  &  \textbf{x1991}      \\
 &      & 10             &  $6.13\pm{0.02}$ ms     &  \textbf{x236}   & $6.13\pm{0.02}$ ms  & \textbf{x666}        \\
 &       & 100            &  $5.43\pm{0.01}$ ms     &  \textbf{x266}   & $5.43\pm{0.01}$ ms  &  \textbf{x752}         \\
 &        & 1000           &  $5.43\pm{0.01}$ ms     &  \textbf{x266}   & $5.43\pm{0.01}$ ms  &  \textbf{x752}       \\
\hline
BIB-AE & GPU   & 1              & $3.14\pm{0.01}$ ms & \textbf{x460}      &  $3.19\pm{0.01}$ ms & \textbf{x1279} \\
 &   & 10              & $1.56\pm{0.01}$ ms & \textbf{x926}      &  $1.57\pm{0.01}$ ms & \textbf{x2600}\\
 &    & 100              & $1.42\pm{0.01}$ ms & \textbf{x1017}      &  $1.42\pm{0.01}$ ms  & \textbf{x2874}\\
%\hline 
%GAN & GPU V100  & 1             & $3.08\pm{0.12}$ ms & \textbf{x793}       &  $3.15\pm{0.12}$ ms & \textbf{x2896}  \\
%GAN & GPU V100  & 10            & $5.21\pm{0.10}$ ms & \textbf{x469}       &  $5.31\pm{0.11}$ ms & \textbf{x1718} \\
%GAN & GPU V100  & 100           & $0.54\pm{0.08}$ ms & \textbf{x4528}      &  $0.65\pm{0.10}$ ms & \textbf{x14039}\\
%GAN & GPU V100  & 1000          & $0.52\pm{0.08}$ ms & \textbf{x4702}      &  $0.64\pm{0.08}$ ms & \textbf{x14258} \\



\hline
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% CONCLUSION 
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusion}

\label{closing}

The accelerated simulation of calorimeters with generative 
deep neural networks is an active area of research. 
Early works~\cite{CaloGAN2,CaloGAN,CaloGAN3} 
established generative networks as a fast and 
very promising tool for particle physics and 
simulated the positron, photon, and charged pion response of an idealised perfect calorimeter with 3 layers
and a total of 504 cells ($3 \times 96$, $12\times 12$, and $12 \times 6$).

Using the WGAN architecture and an energy constrainer network~\cite{ErdmannWGAN2} allowed the correct simulation
of the observed total energy of electrons for a calorimeter consisting of seven layers with a total of 1,260 cells ($12\times 15$ cells per layers). However, a mismodelling of individual cell energies below 10 MIPs, also leading to an observed deviation in the hit multiplicity distribution, was observed and studied. Our implementation of a WGAN based on~\cite{ErdmannWGAN2} reproduces this effect (see Fig.~\ref{fig:results_diffdist1}~(left)).
The proposed BIB-AE architecture with additional MMD loss term and Post Processor Network leads to a reliable description
of low energy deposits.

The ATLAS collaboration also reported the accurate simulation of high-level observables for photons in a four-layer
calorimeter segment with a total of 276 cells ($7 \times 3$, $57 \times 4$, $7\times 7$ and $7 \times 5$) using a VAE architecture~\cite{ATLAS_Gen2}
and 266 cells using a WGAN~\cite{ATLAS_Gen3}.
Recent progress was made applying a GAN architecture to simulating electrons in a high granularity calorimeter prototype~\cite{Sofia}. The considered detector consists of 25~layers with $51\times51$ cells
per layer, leading to a total of 65k cells to be simulated. On this very challenging problem, good agreement with GEANT4 was achieved for a number of differential distributions and correlations of high-level observables. Specifically, the per-cell energy distribution was not reported, however the disagreement in the hit multiplicity again implies a mismodeling of the MIP peak region.

Our specific contribution is the first high fidelity simulation
for a number of challenging quantities relevant for 
downstream analysis, including  the overall energy response and per-cell energy distribution around the MIP peak,
for a realistic high-granularity calorimeter. This is made possible by the first application of the BIB-AE architecture 
--- unifying GAN and VAE approaches --- in physics. Modifications to this architecture, specifically an
additional kernel-based MMD loss term and a Post Processor Network, were developed.
These improvements can potentially also be applied to other generative architectures and models.
Planned future work includes the extension of this approach to also cover
multiple particle types, incident positions and angles towards a complete, fast,
and physically reliable synthetic calorimeter simulation.


==> version_0/4_BIB.tex <==



@article{g4,
title = "{Geant4—a simulation toolkit}",
journal = "Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment",
volume = "506",
number = "3",
pages = "250 - 303",
year = "2003",
issn = "0168-9002",
doi = "https://doi.org/10.1016/S0168-9002(03)01368-8",
url = "http://www.sciencedirect.com/science/article/pii/S0168900203013688",
author = "S. Agostinelli and others"
}

@article{atlas_fastsim,
    author = "Jansky, Roland",
    doi = "10.1088/1742-6596/664/7/072024",
    journal = "J. Phys. Conf. Ser.",
    number = "7",
    pages = "072024",
    title = "{The ATLAS Fast Monte Carlo Production Chain Project}",
    volume = "664",
    year = "2015"
}

@article{ILD-IDR,
    author = "Abramowicz, Halina and others",
    archivePrefix = "arXiv",
    collaboration = "ILD Concept Group",
    eprint = "2003.01116",
    month = "3",
    primaryClass = "physics.ins-det",
    reportNumber = "DESY-20-034, KEK 2019-57",
    title = "{International Large Detector: Interim Design Report}",
    year = "2020"
}

@misc{ilcsoft,
    author ="",
    year = "2016",
    title= "{iLCSoft Project Page}",
    howpublished = "\url{https://github.com/iLCSoft}"
}

@article{dd4hep,
      author         = "Frank, Markus and Gaede, F. and Grefe, C. and Mato, P.",
      title          = "{DD4hep: A Detector Description Toolkit for High Energy
                        Physics Experiments}",
      booktitle      = "{Proceedings, 20th International Conference on Computing
                        in High Energy and Nuclear Physics (CHEP 2013): Amsterdam,
                        The Netherlands, October 14-18, 2013}",
      journal        = "J. Phys. Conf. Ser.",
      volume         = "513",
      year           = "2014",
      pages          = "022010",
      doi            = "10.1088/1742-6596/513/2/022010",
      SLACcitation   = "%%CITATION = 00462,513,022010;%%"
}


@article{early_stuff,
	author         = "Lonnblad, Leif and Peterson, Carsten and Rognvaldsson, Thorsteinn",
	title          = "{Using neural networks to identify jets}",
	journal        = "Nucl. Phys.",  
	volume         = "B349",
	year           = "1991",
	pages          = "675",
	doi            = "10.1016/0550-3213(91)90392-B"
}
	
@article{jet_images,
	author         = "Cogan, Josh and Kagan, Michael and Strauss, Emanuel and Schwarztman, Ariel",
	title          = "{Jet-Images: Computer Vision Inspired Techniques for Jet Tagging}",
	journal        = "JHEP",
	volume         = "1502",
	year           = "2015",
	pages          = "118",
	doi            = "10.1007/JHEP02(2015)118",
	eprint         = "1407.5675",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jet_images2,
	author         = "de Oliveira, Luke and Kagan, Michael and Mackey, Lester and Nachman, Benjamin and Schwartzman, Ariel",
	title          = "{Jet-images — deep learning edition}",
	journal        = "JHEP",
	volume         = "1607",
	year           = "2016",
	pages          = "069",
	doi            = "10.1007/JHEP07(2016)069",
	eprint         = "1511.05190",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{particlenet,
      author         = "Qu, Huilin and Gouskos, Loukas",
      title          = "{ParticleNet: Jet Tagging via Particle Clouds}",
      volume={101},
      ISSN={2470-0029},
      url={http://dx.doi.org/10.1103/PhysRevD.101.056019},
      DOI={10.1103/physrevd.101.056019},
      number={5},
      journal={Physical Review D},
      publisher={American Physical Society (APS)},
      year={2020},
      month={Mar},
      eprint         = "1902.08570",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1902.08570;%%"
}

@article{jedinet,
      author         = "Moreno, Eric A. and Cerri, Olmo and Duarte, Javier M. and
                        Newman, Harvey B. and Nguyen, Thong Q. and Periwal, Avikar
                        and Pierini, Maurizio and Serikova, Aidana and Spiropulu,
                        Maria and Vlimant, Jean-Roch",
      title          = "{JEDI-net: a jet identification algorithm based on
                        interaction networks}",
      journal        = "Eur. Phys. J.",
      volume         = "C80",
      year           = "2020",
      number         = "1",
      pages          = "58",
      doi            = "10.1140/epjc/s10052-020-7608-4",
      eprint         = "1908.05318",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-19-360-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1908.05318;%%"
}

@article{jets_qg,
	author         = "Gallicchio, Jason and Schwartz, Matthew D.",
	title          = "{Quark and Gluon Jet Substructure}",
	journal        = "JHEP",
	volume         = "1304",
	year           = "2013",
	pages          = "090",
	doi            = "10.1007/JHEP04(2013)090",
	eprint         = "1211.7038",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_qg2,
	author         = "Komiske, Patrick T. and Metodiev, Eric M. and Schwartz, Matthew D.",
	title          = "{Deep learning in color: towards automated quark/gluon jet discrimination}",
	journal        = "JHEP",
	volume         = "1701",
	year           = "2017",
	pages          = "110",
	doi            = "10.1007/JHEP01(2017)110",
	eprint         = "1612.01551",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_qg3,
	author         = "Cheng, Taoli",
	title          = "{Recursive Neural Networks in Quark/Gluon Tagging}",
	journal        = "Comput.\ Softw.\ Big Sci.\",
	volume         = "2",
	issue          = "1, 3",
	year           = "2018",
	doi            = "10.1007/s41781-018-0007-y",
	eprint         = "1711.02633",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_qg4,
      author         = "Komiske, Patrick T. and Metodiev, Eric M. and Thaler,
                        Jesse",
      title          = "{Energy Flow Networks: Deep Sets for Particle Jets}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2019",
      pages          = "121",
      doi            = "10.1007/JHEP01(2019)121",
      eprint         = "1810.05165",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP 5064",
      SLACcitation   = "%%CITATION = ARXIV:1810.05165;%%"
}

@article{jets_qg5,
      author         = "Bright-Thonney, Samuel and Nachman, Benjamin",
      title          = "{Investigating the Topology Dependence of Quark and Gluon
                        Jets}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2019",
      pages          = "098",
      doi            = "10.1007/JHEP03(2019)098",
      eprint         = "1810.05653",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1810.05653;%%"
}

@article{lola_qg,
      author         = "Kasieczka, Gregor and Kiefer, Nicholas and Plehn, Tilman
                        and Thompson, Jennifer M.",
      title          = "{Quark-Gluon Tagging: Machine Learning vs Detector}",
      journal        = "SciPost Phys.",
      volume         = "6",
      year           = "2019",
      number         = "6",
      pages          = "069",
      doi            = "10.21468/SciPostPhys.6.6.069",
      eprint         = "1812.09223",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1812.09223;%%"
}

@article{jets_w,
	author         = "Baldi, Pierre and Bauer, Kevin and Eng, Clara and Sadowski, Peter and Whiteson, Daniel",
	title          = "{Jet substructure classification in high-energy physics with deep neural networks}",
	journal        = "Phys. Rev. D",
	volume         = "93",
	issue          = "9",
	year           = "2016",
	pages          = "094034",
	doi            = "10.1103/PhysRevD.93.094034",
	eprint         = "1603.09349",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ex"
}

@article{jets_w2,
	author         = "Louppe, Gilles and Cho, Kyunghyun and Becot, Cyril and Cranmer, Kyle",
	title          = "{QCD-Aware Recursive Neural Networks for Jet Physics}",
	journal        = "JHEP",
	volume         = "1901",
	year           = "2019",
	pages          = "057",
	doi            = "10.1007/JHEP01(2019)057",
	eprint         = "1702.00748",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_h,
      author         = "Lim, Sung Hak and Nojiri, Mihoko M.",
      title          = "{Spectral Analysis of Jet Substructure with Neural
                        Networks: Boosted Higgs Case}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2018",
      pages          = "181",
      doi            = "10.1007/JHEP10(2018)181",
      eprint         = "1807.03312",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KEK-TH-2060",
      SLACcitation   = "%%CITATION = ARXIV:1807.03312;%%"
}

@article{jets_h2,
      author         = "Lin, Joshua and Freytsis, Marat and Moult, Ian and
                        Nachman, Benjamin",
      title          = "{Boosting $H\to b\bar b$ with Machine Learning}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2018",
      pages          = "101",
      doi            = "10.1007/JHEP10(2018)101",
      eprint         = "1807.10768",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1807.10768;%%"
}

@article{deep_top1,
	author         = "Kasieczka, Gregor and Plehn, Tilman and Russell, Michael and Schell, Torben",
	title          = "{Deep-learning Top Taggers or The End of QCD?}",
	journal        = "JHEP",
	volume         = "1705",
	year           = "2017",
	pages          = "006",
	doi            = "10.1007/JHEP05(2017)006",
	eprint         = "1701.08784",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{deep_top2,
	author         = "Macaluso, Sebastian and Shih, David",
	title          = "{Pulling Out All the Tops with Computer Vision and Deep Learning}",
	journal        = "JHEP",
	volume         = "1810",
	year           = "2018",
	pages          = "121",
	doi            = "10.1007/JHEP10(2018)121",
	eprint         = "1803.00107",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}
   
@article{lola,
	author         = "Butter, Anja and Kasieczka, Gregor and Plehn, Tilman and Russell, Michael",
	title          = "{Deep-learned Top Tagging with a Lorentz Layer}",
	journal        = "SciPost Phys.",
	volume         = "5",
	year           = "2018",
	pages          = "028",
	doi            = "10.21468/SciPostPhys.5.3.028",
	eprint         = "1707.08966",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_top,
	author         = "Leandro G. Almeida and Mihailo Backovic and Mathieu Cliche and Seung J. Lee and Maxim Perelstein",
	title          = "{Playing Tag with ANN: Boosted Top Identification with Pattern Recognition}",
	journal        = "JHEP",
	volume         = "1507",
	year           = "2015",
	pages          = "086",
	doi            = "10.1007/JHEP07(2015)086",
	eprint         = "1501.05968",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jets_top2,
      author         = "Pearkes, Jannicke and Fedorko, Wojciech and Lister,
                        Alison and Gay, Colin",
      title          = "{Jet Constituents for Deep Neural Network Based Top Quark
                        Tagging}",
      year           = "2017",
      eprint         = "1704.02124",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1704.02124;%%"
}

@article{jets_top3,
      author         = "Egan, Shannon and Fedorko, Wojciech and Lister, Alison
                        and Pearkes, Jannicke and Gay, Colin",
      title          = "{Long Short-Term Memory (LSTM) networks with jet
                        constituents for boosted top tagging at the LHC}",
      year           = "2017",
      eprint         = "1711.09059",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1711.09059;%%"
}

@article{jets_top4,
      author         = "Choi, Suyong and Lee, Seung J. and Perelstein, Maxim",
      title          = "{Infrared Safety of a Neural-Net Top Tagging Algorithm}",
      journal        = "JHEP",
      volume         = "02",
      year           = "2019",
      pages          = "132",
      doi            = "10.1007/JHEP02(2019)132",
      eprint         = "1806.01263",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1806.01263;%%"
}

@article{jets_top5,
      author         = "Moore, Liam and Nordström, Karl and Varma, Sreedevi and
                        Fairbairn, Malcolm",
      title          = "{Reports of My Demise Are Greatly Exaggerated:
                        $N$-subjettiness Taggers Take On Jet Images}",
      journal        = "SciPost Phys.",
      volume         = "7",
      year           = "2019",
      number         = "3",
      pages          = "036",
      doi            = "10.21468/SciPostPhys.7.3.036",
      eprint         = "1807.04769",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "Nikhef 2018-036 KCL-PH-TH-2018-36 CP3-18-48,
                        NIKHEF-2018-036, KCL-PH-TH-2018-36, CP3-18-48",
      SLACcitation   = "%%CITATION = ARXIV:1807.04769;%%"
}

@article{ml_review,
	  NOTE           = "for a review see",
      author         = "Larkoski, Andrew J. and Moult, Ian and Nachman, Benjamin",
      title          = "{Jet Substructure at the Large Hadron Collider: A Review
                        of Recent Advances in Theory and Machine Learning}",
      journal        = "Phys. Rept.",
      volume         = "841",
      year           = "2020",
      pages          = "1-63",
      doi            = "10.1016/j.physrep.2019.11.001",
      eprint         = "1709.04464",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1709.04464;%%"
}

@article{jets_comparison,
      author         = "Kasieczka, Gregor and Plehn, Tilman and others",
      title          = "{The Machine Learning Landscape of Top Taggers}",
      journal        = "SciPost Phys.",
      volume         = "7",
      year           = "2019",
      pages          = "014",
      doi            = "10.21468/SciPostPhys.7.1.014",
      eprint         = "1902.09914",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1902.09914;%%"
}

@article{bayes,
      author         = "Bollweg, Sven and Haußmann, Manuel and Kasieczka, Gregor
                        and Luchmann, Michel and Plehn, Tilman and Thompson,
                        Jennifer",
      title          = "{Deep-Learning Jets with Uncertainties and More}",
      journal        = "SciPost Phys.",
      volume         = "8",
      year           = "2020",
      number         = "1",
      pages          = "006",
      doi            = "10.21468/SciPostPhys.8.1.006",
      eprint         = "1904.10004",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1904.10004;%%"
}

@article{bayes2,
      author         = "Kasieczka, Gregor and Luchmann, Michel and Otterpohl,
                        Florian and Plehn, Tilman",
      title          = "{Per-Object Systematics using Deep-Learned Calibration}",
      year           = "2020",
      eprint         = "2003.11099",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:2003.11099;%%"
}

@article{disco,
      author         = "Kasieczka, Gregor and Shih, David",
      title          = "{DisCo Fever: Robust Networks Through Distance
                        Correlation}",
      year           = "2020",
      eprint         = "2001.05310",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:2001.05310;%%"
}

@article{ben_unc,
      author         = "Nachman, Benjamin",
      title          = "{A guide for deploying Deep Learning in LHC searches: How
                        to achieve optimality and account for uncertainty}",
      year           = "2019",
      eprint         = "1909.03081",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1909.03081;%%"
}

@article{badger,
      author         = "Badger, Simon and Bullock, Joseph",
      title          = "{Using neural networks for efficient evaluation of high
                        multiplicity scattering amplitudes}",
      year           = "2020",
      eprint         = "2002.07516",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IPPP/20/5",
      SLACcitation   = "%%CITATION = ARXIV:2002.07516;%%"
}

@article{bad,
	author         = "Englert, Christoph and Galler, Peter and Harris, Philip and Spannowsky, Michael",
	title          = "{Machine Learning Uncertainties with Adversarial Neural Networks}",
	journal        = "Eur. Phys. J.",
	volume         = "C79",
	issue          = "1, 4",
	year           = "2019",
	doi            = "10.1140/epjc/s10052-018-6511-8",
	eprint         = "1807.08763",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{aussies,
	author         = "Barnard, James and Dawe, Edmund Noel and Dolan, Matthew J. and Rajcic, Nina",
	title          = "{Parton Shower Uncertainties in Jet Substructure Analyses with Deep Neural Networks}",
	journal        = "Phys. Rev. D",
	volume         = "95",
	issue          = "1",
	year           = "2017",
	pages          = "014018",
	doi            = "10.1103/PhysRevD.95.014018",
	eprint         = "1609.00607",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@incollection{pivot,
      title = "{Learning to Pivot with Adversarial Networks}",
      author = {Louppe, Gilles and Kagan, Michael and Cranmer, Kyle},
      booktitle = {Advances in Neural Information Processing Systems 30},
      editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
      pages = {981--990},
      year = {2017},
      publisher = {Curran Associates, Inc.},
      url = {http://papers.nips.cc/paper/6699-learning-to-pivot-with-adversarial-networks.pdf},
      eprint         = "1611.01046",
      archivePrefix  = "arXiv",
      primaryClass   = "stat.ML",
      SLACcitation   = "%%CITATION = ARXIV:1611.01046;%%"
}

@article{weak,
	author         = "Dery, Lucio Mwinmaarong and Nachman, Benjamin and Rubbo, Francesco and Schwartzman, Ariel",
	title          = "{Weakly Supervised Classification in High Energy Physics}",
	journal        = "JHEP",
	volume         = "1705",
	year           = "2017",
	pages          = "145",
	doi            = "10.1007/JHEP05(2017)145",
	eprint         = "1702.00414",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{weak2,
	author         = "Cohen, Timothy and Freytsis, Marat and Ostdiek, Bryan",
	title          = "{(Machine) Learning to Do More with Less}",
	journal        = "JHEP",
	volume         = "1802",
	year           = "2018",
	pages          = "034",
	doi            = "10.1007/JHEP02(2018)034",
	eprint         = "1706.09451",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{weak3,
	author         = "Metodiev, Eric M. and Nachman, Benjamin and Thaler, Jesse",
	title          = "{Classification without labels: Learning from mixed samples in high energy physics}",
	journal        = "JHEP",
	volume         = "1710",
	year           = "2017",
	pages          = "174",
	doi            = "10.1007/JHEP10(2017)174",
	eprint         = "1708.02949",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{weak4,
	author         = "Komiske, Patrick T. and Metodiev, Eric M. and Nachman, Benjamin and Schwartz, Matthew D.",
	title          = "{Learning to classify from impure samples with high-dimensional data}",
	journal        = "Phys. Rev. D",
	volume         = "98",
	issue          = "1",
	year           = "2018",
	pages          = "011502",
	doi            = "10.1103/PhysRevD.98.011502",
	eprint         = "1801.10158",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{weak5,
      author         = "Andreassen, Anders and Feige, Ilya and Frye, Christopher
                        and Schwartz, Matthew D.",
      title          = "{JUNIPR: a Framework for Unsupervised Machine Learning in
                        Particle Physics}",
      journal        = "Eur. Phys. J.",
      volume         = "C79",
      year           = "2019",
      number         = "2",
      pages          = "102",
      doi            = "10.1140/epjc/s10052-019-6607-9",
      eprint         = "1804.09720",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1804.09720;%%"
}

@article{weak6,
      author         = "Heimel, Theo and Kasieczka, Gregor and Plehn, Tilman and
                        Thompson, Jennifer M.",
      title          = "{QCD or What?}",
      journal        = "SciPost Phys.",
      volume         = "6",
      year           = "2019",
      number         = "3",
      pages          = "030",
      doi            = "10.21468/SciPostPhys.6.3.030",
      eprint         = "1808.08979",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1808.08979;%%"
}

@article{weak7,
    author = "Farina, Marco and Nakai, Yuichiro and Shih, David",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.101.075021",
    eprint = "1808.08992",
    journal = "Phys. Rev. D",
    number = "7",
    pages = "075021",
    primaryClass = "hep-ph",
    title = "{Searching for New Physics with Deep Autoencoders}",
    volume = "101",
    year = "2020",
    SLACcitation   = "%%CITATION = ARXIV:1808.08992;%%"
}
@article{weak8,
      author         = "Cerri, Olmo and Nguyen, Thong Q. and Pierini, Maurizio
                        and Spiropulu, Maria and Vlimant, Jean-Roch",
      title          = "{Variational Autoencoders for New Physics Mining at the
                        Large Hadron Collider}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2019",
      pages          = "036",
      doi            = "10.1007/JHEP05(2019)036",
      eprint         = "1811.10276",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1811.10276;%%"
}

@article{koalahunting,
      author         = "Collins, Jack H. and Howe, Kiel and Nachman, Benjamin",
      title          = "{Anomaly Detection for Resonant New Physics with Machine
                        Learning}",
      journal        = "Phys. Rev. Lett.",
      volume         = "121",
      year           = "2018",
      number         = "24",
      pages          = "241803",
      doi            = "10.1103/PhysRevLett.121.241803",
      eprint         = "1805.02664",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-18-180-T",
      SLACcitation   = "%%CITATION = ARXIV:1805.02664;%%"
}

@article{tagntrain,
      author         = "Amram, Oz and Suarez, Cristina Mantilla",
      title          = "{Tag N' Train: A Technique to Train Improved Classifiers
                        on Unlabeled Data}",
      year           = "2020",
      eprint         = "2002.12376",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:2002.12376;%%"
}

@article{ANODE,
  title = "{Anomaly detection with density estimation}",
  author = {Nachman, Benjamin and Shih, David},
  journal = {Phys. Rev. D},
  volume = {101},
  issue = {7},
  pages = {075042},
  numpages = {16},
  year = {2020},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.101.075042},
  eprint={2001.04990},
  archivePrefix={arXiv},
  primaryClass={hep-ph}
}

@article{capsules,
      author         = "Diefenbacher, Sascha and Frost, Hermann and Kasieczka,
                        Gregor and Plehn, Tilman and Thompson, Jennifer M.",
      title          = "{CapsNets Continuing the Convolutional Quest}",
      journal        = "SciPost Phys.",
      volume         = "8",
      year           = "2020",
      pages          = "023",
      doi            = "10.21468/SciPostPhys.8.2.023",
      eprint         = "1906.11265",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1906.11265;%%"
}}

@article{information,
	author         = "Datta, Kaustuv and Larkoski, Andrew",
	title          = "{How Much Information is in a Jet?}",
	journal        = "JHEP",
	volume         = "1706",
	year           = "2017",
	pages          = "073",
	doi            = "10.1007/JHEP06(2017)073",
	eprint         = "1704.08249",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{information2,
	author         = "Chang, Spencer and Cohen, Timothy and Ostdiek, Bryan",
	title          = "{What is the Machine Learning?}",
	journal        = "Phys. Rev. D ",
	volume         = "97",
	issue          = "5",
	year           = "2018",
	pages          = "056009",
	doi            = "10.1103/PhysRevD.97.056009",
	eprint         = "1709.10106",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{information3,
	author         = "Datta, Kaustuv and Larkoski, Andrew J.",
	title          = "{Novel Jet Observables from Machine Learning}",
	journal        = "JHEP",
	volume         = "1803",
	year           = "2018",
	pages          = "086",
	doi            = "10.1007/JHEP03(2018)086",
	eprint         = "1710.01305",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{information4,
	author         = "Komiske, Patrick T. and Metodiev, Eric M. and Thaler, Jesse",
	title          = "{Energy flow polynomials: A complete linear basis for jet substructure}",
	journal        = "JHEP",
	volume         = "1804",
	year           = "2018",
	pages          = "013",
	doi            = "10.1007/JHEP04(2018)013",
	eprint         = "1712.07124",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{information5,
	author         = "Thomas Roxlo and Matthew Reece",
	title          = "{Opening the black box of neural nets: case studies in stop/top discrimination}",
	eprint         = "1804.09278",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{qjets,
	NOTE           = "for some ideas on uncertainties in jet classification see",
	author         = "Ellis, Stephen D. and Hornig, Andrew and Krohn, David and Roy, Tuhin S.",
	title          = "{On Statistical Aspects of Qjets}",
	journal        = "JHEP",
	volume         = "1501",
	year           = "2015",
	pages          = "022",
	doi            = "10.1007/JHEP01(2015)022",
	eprint         = "1409.6785",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{qjets2,
	NOTE           = "for some ideas on uncertainties in jet classification see",
	author         = "Mackey, Lester and Nachman, Benjamin and Schwartzman, Ariel and Stansbury, Conrad",
	title          = "{Fuzzy Jets}",
	journal        = "JHEP",
	volume         = "1606",
	year           = "2016",
	pages          = "010",
	doi            = "10.1007/JHEP06(2016)010",
	eprint         = "1509.02216",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{medical,
	NOTE           = "for a similar study in a different field see",
	author         = "Leibig, Christian and Allken, Vaneeda and Ayhan, Murat Seckin and Berens, Phillip and Wahl, Siegfried",
	title          = "{Leveraging uncertainty information from deep neural networks for disease detection}",
	journal        = "Scientific Reports",
	volume         = "7",
	year           = "2017",
	pages          = "17816 ",
	doi            = "10.1038/s41598-017-17876-z",
}

@article{deep_errors,
	author         = "Alex Kendall and Yarin Gal",
	title          = "{What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?}",
	journal        = "Proc. NIPS",
	year           = "2017",
	eprint         = "1703.04977",
    archivePrefix  = "arXiv",
    primaryClass   = "cs.CV"
}

@article{bnn_early,
	author         = "MacKay, David",
	title          = "{Probable Networks and Plausible Predictions – A Review of Practical Bayesian Methods for Supervised Neural Networks}",
	journal        = "Comp. in Neural Systems",
	volume         = "6",
	year           = "1995",
	pages          = "4679",
	url            = {http://www.inference.org.uk/mackay/network.pdf}
}

@phdthesis{bnn_early2,
    author       = "Neal, Radford M.", 
    title        = "{Bayesian learning for neural networks}",
    school       = "Toronto",
    year         = "1995",
    url          = {ftp://www.cs.toronto.edu/dist/radford/thesis.pdf}
}

@phdthesis{bnn_early3,
    author       = "Gal, Yarin", 
    title        = "{Uncertainty in Deep Learning}",
    school       = "Cambridge",
    year         = "2016",
    url          = {http://mlg.eng.cam.ac.uk/yarin/thesis/thesis.pdf}
}

@article{bnn_tev,
	author         = "Bhat, Pushpalatha C. and Prosper, Harrison B.",
	title          = "{Bayesian neural networks}",
	journal        = "Conf. Proc. C",
	volume         = "050912",
	year           = "2005",
	pages          = "151",
	url            = {http://www.physics.ox.ac.uk/phystat05/proceedings/files//bhat_prosper_phystat05.pdf}
}

@mastersthesis{bnn_tev2,
	author         = "Saucedo, Skyler Richard",
	title          = "{Bayesian Neural Networks for Classification}",
	school         = "Florida State University",
	year           = "2007",
	url            = {http://purl.flvc.org/fsu/fd/FSU_migr_etd-2069}
}

@article{bnn_nu,
	author         = "Xu, Ye and Xu, Weiwei and Meng, Yixiong and Zhu, Kaien and Xu, Wei",
	title          = "{Applying Bayesian Neural Networks to Event Reconstruction in Reactor Neutrino Experiments}",
	journal        = "Nucl. Instrum. Meth. A",
	volume         = "592",
	year           = "2008",
	pages          = "451",
	doi            = "10.1016/j.nima.2008.04.006",
	eprint         = "0712.4042",
    archivePrefix  = "arXiv",
    primaryClass   = "physics.data-an"
}

@article{blei,
	author         = "Blei, David M. and Kucukelbir, Alp and McAuliffe, Jon D.",
	title          = "{Variational Inference: A Review for Statisticians}",
	journal        = "JASA",
	volume         = "112",
	year           = "2017",
	pages          = "859",
	doi            = "10.1080/01621459.2017.1285773",
	eprint         = "1601.00670",
    archivePrefix  = "arXiv",
    primaryClass   = "stat.CO"
}

@article{tensorflow_probability,
	author         = "Abadi, Martin and others",
	title          = "{TensorFlow: A System for Large-Scale Machine Learning}",
	journal        = "OSDI",
	volume         = "16",
	year           = "2016",
	pages          = "265",
	url            = "https://www.tensorflow.org/probability"
}

@article{flipout,
	author         = "Yeming Wen and Paul Vicol and Jimmy Ba and Dustin Tran and Roger Grosse",
	title          = "{Method for calculating gradients}",
	journal        = "Proc. NIPS",
	year           = "2018",
	eprint         = "1803.04386",
  archivePrefix  = "arXiv",
  primaryClass   = "cs.LG"
}

@article{adam,
  author    = {Diederik P. Kingma and
               Jimmy Ba},

  title     = "{Adam: {A} Method for Stochastic Optimization}",
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015},
  year      = {2015},
  eprint    = "1412.6980",
  archivePrefix  = "arXiv",
  primaryClass   = "cs.LG",
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{pythia,
	author         = "Sj{\"o}strand, Torbj{\"o}rn and others",
	title          = "{An Introduction to PYTHIA 8.2}",
	journal        = "Comput. Phys. Commun.",
	volume         = "191",
	year           = "2015",
	pages          = "159",
	doi            = "10.1016/j.cpc.2015.01.024",
	eprint         = "1410.3012",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{delphes,
	author         = "de Favereau, J. and Delaere, C. and Demin, P. and Giammanco, A. and Lemaitre, V. and Mertens, A. and Selvaggi, M.",
	title          = "{DELPHES 3, A modular framework for fast simulation of a generic collider experiment}",
	collaboration  = "DELPHES 3 Collaboration",
	journal        = "JHEP",
	volume         = "1402",
	year           = "2014",
	pages          = "057",
	doi            = "10.1007/JHEP02(2014)057",
	eprint         = "1307.6346",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ex"
}

@article{anti_kt,
	author         = "Cacciari, Matteo and Salam, Gavin P and Soyez, Gregory",
	title          = "{The Anti-k(t) jet clustering algorithm}",
	collaboration  = "DELPHES 3 Collaboration",
	journal        = "JHEP",
	volume         = "0804",
	year           = "2008",
	pages          = "063",
	doi            = "10.1088/1126-6708/2008/04/063",
	eprint         = "0802.1189",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}
  
@article{fastjet,
	author         = "Cacciari, Matteo and Salam, Gavin P.",
	title          = "{Dispelling the $N^{3}$ myth for the $k_t$ jet-finder}",
	collaboration  = "DELPHES 3 Collaboration",
	journal        = "Phys. Lett.  B",
	volume         = "641",
	year           = "2006",
	pages          = "57",
	doi            = "10.1016/j.physletb.2006.08.037",
	eprint         = "0512210",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{fastjet2,
	author         = "Cacciari, Matteo and Salam, Gavin P. and Soyez, Gregory",
	title          = "{FastJet User Manual}",
	collaboration  = "DELPHES 3 Collaboration",
	journal        = "Eur. Phys. J. C",
	volume         = "1896",
	year           = "2012",
	doi            = "10.1140/epjc/s10052-012-1896-2",
	eprint         = "1111.6097",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{recalibrate,
	author         = "Chuan Guo and Geoff Pleiss and Yu Sun and Kilian Q. Weinberger",
	title          = "{On Calibration of Modern Neural Networks}",
	collaboration  = "DELPHES 3 Collaboration",
	journal        = "Proc. ICML",
	year           = "2017",
	eprint         = "1706.04599",
    archivePrefix  = "arXiv",
    primaryClass   = "cs.LG"
}

@article{platt_scaling,
	author         = "Platt, John C.",
	title          = "{Probabilistic outputs for support vector machines and comparisons to regularized likelihood methods}",
	journal        = "Adv. Large Margin Classifiers",
	volume         = "10(3)",
	year           = "1999",
	pages          = "61"	
}

@article{dropout,
	author         = "Geoffrey E. Hinton and Nitish Srivastava and Alex Krizhevsky and Ilya Sutskever and Ruslan R. Salakhutdinov",
	title          = "{Improving neural networks by preventing co-adaptation of feature detectors}",
	eprint         = "1207.0580",
    archivePrefix  = "arXiv",
    primaryClass   = "cs.NE"
}

@article{dropout_equiv,
	author         = "Yarin Gal and Zoubin Ghahramani",
	title          = "{Dropout as a Bayesian Approximation: Representing Model Uncertainty in Deep Learning }",
	journal        = "Proc. ICML",
	year           = "2016",
	eprint         = "1506.02142",
    archivePrefix  = "arXiv",
    primaryClass   = "stat.ML"
}

@article{top_review,
	author         = "Plehn, Tilman and Spannowsky, Michael",
	title          = "{Top Tagging}",
	journal        = "J. Phys. G ",
	volume         = "39",
	year           = "2012",
	pages          = "083001",
	doi            = "10.1088/0954-3899/39/8/083001",
	eprint         = "1112.4441",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{jes,
	author         = "Khachatryan, V. and Sirunyan, A.M. and Tumasyan, A. and Adam, W. and Asilar, E. and Bergauer, T. and Brandstetter, J. and Brondolin, E. and Dragicevic, M. and Erö, J. and others",
	title          = "{Jet energy scale and resolution in the CMS experiment in pp collisions at 8 TeV}",
	collaboration  = "CMS Collaboration",
	journal        = "JINST",
	volume         = "12",
	issue          = "02",
	year           = "2017",
	pages          = "P02014",
	doi            = "10.1088/1748-0221/12/02/P02014",
	eprint         = "1607.03663",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ex"
}

@article{jes2,
	author         = "Aaboud, M. and Aad, G. and Abbott, B. and Abdallah, J. and Abdinov, O. and Abeloos, B. and Abidi, S. H. and AbouZeid, O. S. and Abraham, N. L. and Abramowicz, H. and others",
	title          = "{Jet energy scale measurements and their systematic uncertainties in proton-proton collisions at $\sqrt{s} = 13$ TeV with the ATLAS detector}",
	collaboration  = "ATLAS Collaboration",
	journal        = "Phys. Rev. D",
	volume         = "96",
	issue          = "7",
	year           = "2017",
	pages          = "072002",
	doi            = "10.1103/PhysRevD.96.072002",
	eprint         = "1703.09665",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ex"
}

@article{adv_ex,
	author         = "Goodfellow, Ian J. and Shlens, Jonathon and Szegedy, Christian",
	title          = "{Explaining and Harnessing Adversarial Examples}",
	eprint         = "1412.6572",
    archivePrefix  = "arXiv",
    primaryClass   = "stat.ML"
}

@article{puppi,
	author         = "Bertolini, Daniele and Harris, Philip and Low, Matthew and Tran, Nhan",
	title          = "{Pileup Per Particle Identification}",
	journal        = "JHEP",
	volume         = "1410",
	year           = "2014",
	pages          = "059",
	doi            = "10.1007/JHEP10(2014)059",
	eprint         = "1407.6013",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{softkiller,
	author         = "Cacciari, Matteo and Salam, Gavin P. and Soyez, Gregory",
	title          = "{SoftKiller, a particle-level pileup removal method}",
	journal        = "Eur. Phys. J. C",
	volume         = "75",
	issue          = "2",
	year           = "2015",
	pages          = "59",
	doi            = "10.1140/epjc/s10052-015-3267-2",
	eprint         = "1407.0408",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{MLpileup,
	author         = "P.~T.~Komiske, E.~M.~Metodiev, B.~Nachman and M.~D.~Schwartz",
	title          = "{Pileup Mitigation with Machine Learning (PUMML)}",
	journal        = "JHEP",
	volume         = "1712",
	year           = "2017",
	pages          = "051",
	doi            = "10.1007/JHEP12(2017)051",
	eprint         = "1707.08600",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}

@article{MLpileup2,
      author         = "Arjona Martínez, J. and Cerri, Olmo and Pierini,
                        Maurizio and Spiropulu, Maria and Vlimant, Jean-Roch",
      title          = "{Pileup mitigation at the Large Hadron Collider with
                        graph neural networks}",
      journal        = "Eur. Phys. J. Plus",
      volume         = "134",
      year           = "2019",
      number         = "7",
      pages          = "333",
      doi            = "10.1140/epjp/i2019-12710-3",
      eprint         = "1810.07988",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1810.07988;%%"
}

@article{heptop,
	author         = "Plehn, Tilman and Spannowsky, Michael and Takeuchi, Michihisa and Zerwas, Dirk",
	title          = "{Stop Reconstruction with Tagged Tops}",
	journal        = "JHEP",
	volume         = "1010",
	year           = "2010",
	pages          = "078",
	doi            = "10.1007/JHEP10(2010)078",
	eprint         = "1006.2833",
    archivePrefix  = "arXiv",
    primaryClass   = "hep-ph"
}


@article{DeepJet,
      title         = "{Performance of the DeepJet b tagging algorithm using
                       41.9/fb of data from proton-proton collisions at 13TeV with
                       Phase 1 CMS detector}",      
      author        = "{CMS Collaboration}",
      month         = "Nov",
      year          = "2018",
      journal  = "CMS-DP-2018-058",
      url           = "http://cds.cern.ch/record/2646773",
}

@article{CMSTop,      
      collaboration  = "{CMS Collaboration}",
      title          = "{Machine learning-based identification of highly
                        Lorentz-boosted hadronically decaying particles at the CMS
                        experiment}",
      year           = "2019",
      journal   = "CMS-PAS-JME-18-002",
      url           = "https://cds.cern.ch/record/2683870",

      SLACcitation   = "%%CITATION = CMS-PAS-JME-18-002;%%"
}

@article{ATLASTop,
      author={Aaboud, M. and others},      
      collaboration  = "{ATLAS Collaboration}",
      title          = "{Performance of top-quark and $W$-boson tagging with
                        ATLAS in Run 2 of the LHC}",      
      journal        = "Eur. Phys. J.",
      volume         = "C79",
      year           = "2019",
      number         = "5",
      pages          = "375",
      doi            = "10.1140/epjc/s10052-019-6847-8",
      eprint         = "1808.07858",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-EP-2018-192",
      SLACcitation   = "%%CITATION = ARXIV:1808.07858;%%"
}

@techreport{ATLASCorrelation,
      title         = "{Performance of mass-decorrelated jet substructure
                       observables for hadronic two-body decay tagging in ATLAS}",
      institution   = "CERN",
      author        = "{ATLAS Collaboration}",
      address       = "Geneva",
      number        = "ATL-PHYS-PUB-2018-014",
      month         = "Jul",
      year          = "2018",
      reportNumber  = "ATL-PHYS-PUB-2018-014",
      url           = "http://cds.cern.ch/record/2630973",
}


@article{CaloGAN,
      author         = "de Oliveira, Luke and Paganini, Michela and Nachman,
                        Benjamin",
      title          = "{Learning Particle Physics by Example: Location-Aware
                        Generative Adversarial Networks for Physics Synthesis}",
      journal        = "Comput. Softw. Big Sci.",
      volume         = "1",
      year           = "2017",
      number         = "1",
      pages          = "4",
      doi            = "10.1007/s41781-017-0004-6",
      eprint         = "1701.05927",
      archivePrefix  = "arXiv",
      primaryClass   = "stat.ML",
      SLACcitation   = "%%CITATION = ARXIV:1701.05927;%%"
}

@article{CaloGAN2,
      author         = "Paganini, Michela and de Oliveira, Luke and Nachman,
                        Benjamin",
      title          = "{Accelerating Science with Generative Adversarial
                        Networks: An Application to 3D Particle Showers in
                        Multilayer Calorimeters}",
      journal        = "Phys. Rev. Lett.",
      volume         = "120",
      year           = "2018",
      number         = "4",
      pages          = "042003",
      doi            = "10.1103/PhysRevLett.120.042003",
      eprint         = "1705.02355",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1705.02355;%%"
}

@article{CaloGAN3,
      author         = "Paganini, Michela and de Oliveira, Luke and Nachman,
                        Benjamin",
      title          = "{CaloGAN : Simulating 3D high energy particle showers in
                        multilayer electromagnetic calorimeters with generative
                        adversarial networks}",
      journal        = "Phys. Rev.",
      volume         = "D97",
      year           = "2018",
      number         = "1",
      pages          = "014021",
      doi            = "10.1103/PhysRevD.97.014021",
      eprint         = "1712.10321",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1712.10321;%%"
}

@article{ErdmannWGAN,
      author         = "Erdmann, Martin and Geiger, Lukas and Glombitza, Jonas
                        and Schmidt, David",
      title          = "{Generating and refining particle detector simulations
                        using the Wasserstein distance in adversarial networks}",
      journal        = "Comput. Softw. Big Sci.",
      volume         = "2",
      year           = "2018",
      number         = "1",
      pages          = "4",
      doi            = "10.1007/s41781-018-0008-x",
      eprint         = "1802.03325",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1802.03325;%%"
}

@article{ErdmannWGAN2,
      author         = "Erdmann, Martin and Glombitza, Jonas and Quast, Thorben",
      title          = "{Precise simulation of electromagnetic calorimeter
                        showers using a Wasserstein Generative Adversarial
                        Network}",
      journal        = "Comput. Softw. Big Sci.",
      volume         = "3",
      year           = "2019",
      number         = "1",
      pages          = "4",
      doi            = "10.1007/s41781-018-0019-7",
      eprint         = "1807.01954",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1807.01954;%%"
}


@techreport{ATLAS_Gen,
      title         = "{Deep generative models for fast shower simulation in
                       ATLAS}",
      institution   = "CERN",
      author = "{ATLAS Collaboration}",
      address       = "Geneva",
      number        = "ATL-SOFT-PUB-2018-001",
      month         = "Jul",
      year          = "2018",
      reportNumber  = "ATL-SOFT-PUB-2018-001",
      url           = "http://cds.cern.ch/record/2630433",
}

@techreport{ATLAS_Gen2,
      title         = "{VAE for photon shower simulation in ATLAS}",
      institution   = "CERN",
      author = "{ATLAS Collaboration}",
      number        = "ATL-SOFT-SIM-2019-007",
      month         = "October",
      year          = "2019",
      reportNumber  = "ATL-SOFT-SIM-2019-007",
      url           = "https://atlas.web.cern.ch/Atlas/GROUPS/PHYSICS/PLOTS/SIM-2019-007/",
}

@article{ATLAS_Gen3,
      author        = "Ghosh, Aishik",
      title         = "{Deep generative models for fast shower simulation in ATLAS}",
      institution   = "CERN",
      collaboration = "ATLAS Collaboration",
      address       = "Geneva",
      number        = "ATL-SOFT-PROC-2019-007",
      month         = "Jun",
      year          = "2019",
      journal       = "19th International Workshop on Advanced Computing and Analysis Techniques in Physics Research, Saas Fee, Switzerland, 2019",
      reportNumber  = "ATL-SOFT-PROC-2019-007",
      url           = "https://cds.cern.ch/record/2680531",
}

@article{GAN_arxiv,
    title="{Generative Adversarial Networks}",
    author={Ian J. Goodfellow and Jean Pouget-Abadie and Mehdi Mirza and Bing Xu and David Warde-Farley and Sherjil Ozair and Aaron Courville and Yoshua Bengio},
    year={2014},
    eprint={1406.2661},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{GAN, 
    author = {Goodfellow, Ian J. and others}, 
    title = "{Generative Adversarial Nets}", 
    year = {2014},
    address = {Cambridge, MA, USA}, 
    booktitle = {Proceedings of the 27th International Conference on Neural Information Processing Systems - Volume 2},
    pages = {2672–2680}, 
    numpages = {9}, 
    location = {Montreal, Canada}, 
    series = {NIPS’14},
    URL={https://dl.acm.org/doi/10.5555/2969033.2969125},
    eprint={1406.2661},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{StyleGAN,
author = {Karras, Tero and Laine, Samuli and Aila, Timo},
booktitle={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},  
title="{A Style-Based Generator Architecture for Generative Adversarial Networks}",
year = {2019},
month = {06},
pages = {4396-4405},
doi = {10.1109/CVPR.2019.00453},
    eprint={1812.04948},
    archivePrefix={arXiv},
    primaryClass={cs.NE}
}

@article{Conditional,
    title="{Conditional Generative Adversarial Nets}",
    author={Mehdi Mirza and Simon Osindero},
    year={2014},
    eprint={1411.1784},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{WGAN,
    title="{Wasserstein GAN}",
    author={Martin Arjovsky and Soumith Chintala and Léon Bottou},
    year={2017},
    eprint={1701.07875},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{WGAN2,
    title="{Improved Training of Wasserstein GANs}",
    author={Ishaan Gulrajani and Faruk Ahmed and Martin Arjovsky and Vincent Dumoulin and Aaron Courville},
    booktitle = {Advances in Neural Information Processing Systems 30},
    pages = {5767--5777},
    year = {2017},
    url = {http://papers.nips.cc/paper/7159-improved-training-of-wasserstein-gans.pdf},
    eprint={1704.00028},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{VAE,
    title="{Auto-Encoding Variational Bayes}",
    author={Diederik P Kingma and Max Welling},
    year={2013},
    eprint={1312.6114},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@article{BIB-AE,
    title="{Information bottleneck through variational glasses}",
    author={Slava Voloshynovskiy and Mouad Kondah and Shideh Rezaeifar and Olga Taran and Taras Holotyak and Danilo Jimenez Rezende},
    year={2019},
    eprint={1912.00830},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@article{AAE,
    title="{Adversarial Autoencoders}",
    author={Alireza Makhzani and Jonathon Shlens and Navdeep Jaitly and Ian Goodfellow and Brendan Frey},
    year={2015},
    eprint={1511.05644},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{NICE,
    title="{NICE: Non-linear Independent Components Estimation}",
    author={Laurent Dinh and David Krueger and Yoshua Bengio},
    year={2014},
    eprint={1410.8516},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{RealNVP,
    title="{Density estimation using Real NVP}",
    author={Laurent Dinh and Jascha Sohl-Dickstein and Samy Bengio},
    year={2016},
    eprint={1605.08803},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{papamakarios2019normalizing,
    title="{Normalizing Flows for Probabilistic Modeling and Inference}",
    author={George Papamakarios and Eric Nalisnick and Danilo Jimenez Rezende and Shakir Mohamed and Balaji Lakshminarayanan},
    year={2019},
    eprint={1912.02762},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{rezende2015variational,
    title="{Variational Inference with Normalizing Flows}",
    author={Danilo Jimenez Rezende and Shakir Mohamed},
    year={2015},
    booktitle = {Proceedings of the 32nd International Conference on International Conference on Machine Learning - Volume 37}, 
    pages = {1530–1538}, 
    numpages = {9}, 
    location = {Lille, France}, 
    series = {ICML’15},
    eprint={1505.05770},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@article{Sofia,
      author         = "Belayneh, Dawit and others",
      title          = "{Calorimetry with Deep Learning: Particle Simulation and
                        Reconstruction for Collider Physics}",
      year           = "2019",
      eprint         = "1912.06794",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1912.06794;%%"
}

@book{optimal_transport,
    place={Berlin}, 
    title="{Optimal Transport: Old and New}", 
    publisher={Springer, Berlin}, 
    author={Villani C\'edric},
    year={2009}
}

@techreport{hgcal_tdr,
      author        = "{CMS Collaboration}",
      title         = "{The Phase-2 Upgrade of the CMS Endcap Calorimeter}",
      institution   = "CERN",
      address       = "Geneva",
      number        = "CERN-LHCC-2017-023. CMS-TDR-019",
      month         = "Nov",
      year          = "2017",
      reportNumber  = "CERN-LHCC-2017-023",
      url           = "https://cds.cern.ch/record/2293646",
}

@article{CaloGraphs,
    author = "Qasim, Shah Rukh and Kieseler, Jan and Iiyama, Yutaro and Pierini, Maurizio",
    archivePrefix = "arXiv",
    doi = "10.1140/epjc/s10052-019-7113-9",
    eprint = "1902.07987",
    journal = "Eur. Phys. J. C",
    number = "7",
    pages = "608",
    primaryClass = "physics.data-an",
    title = "{Learning representations of irregular particle-detector geometry with distance-weighted graph networks}",
    volume = "79",
    year = "2019"
}

@article{Parametrised,
    author = "Baldi, Pierre and Cranmer, Kyle and Faucett, Taylor and Sadowski, Peter and Whiteson, Daniel",
    archivePrefix = "arXiv",
    doi = "10.1140/epjc/s10052-016-4099-4",
    eprint = "1601.07913",
    journal = "Eur. Phys. J. C",
    number = "5",
    pages = "235",
    primaryClass = "hep-ex",
    title = "{Parameterized neural networks for high-energy physics}",
    volume = "76",
    year = "2016"
}

@article{VAE-GAN,
    title="{Autoencoding beyond pixels using a learned similarity metric}",
    author={Anders Boesen Lindbo Larsen and Søren Kaae Sønderby and Hugo Larochelle and Ole Winther},
    year={2015},
    eprint={1512.09300},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{InfoVAE,
    title="{InfoVAE: Information Maximizing Variational Autoencoders}",
    author={Shengjia Zhao and Jiaming Song and Stefano Ermon},
    year={2017},
    eprint={1706.02262},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{LHCGAN,
    author = "Butter, Anja and Plehn, Tilman and Winterhalder, Ramon",
    archivePrefix = "arXiv",
    doi = "10.21468/SciPostPhys.7.6.075",
    eprint = "1907.03764",
    journal = "SciPost Phys.",
    number = "6",
    pages = "075",
    primaryClass = "hep-ph",
    title = "{How to GAN LHC Events}",
    volume = "7",
    year = "2019"
}


@article{MMD_base,
  author    = {Arthur Gretton and
               Karsten M. Borgwardt and
               Malte J. Rasch and
               Bernhard Sch{\"{o}}lkopf and
               Alexander J. Smola},
  title     = "{A Kernel Method for the Two-Sample Problem}",
  journal   = {CoRR},
  year      = {2008},
  archivePrefix = {arXiv},
  primaryClass={cs.LG},
  eprint    = {0805.2368},
  timestamp = {Mon, 13 Aug 2018 16:47:18 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-0805-2368.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{pytorch,
title = "{PyTorch: An Imperative Style, High-Performance Deep Learning Library}",
author = {Paszke, Adam and others},
journal = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf}
}


@article{PandolfiGAN,
   title="{Fast and Accurate Simulation of Particle Detectors Using Generative Adversarial Networks}",
   volume={2},
   ISSN={2510-2044},
   url={http://dx.doi.org/10.1007/s41781-018-0015-y},
   number={1},
   journal={Computing and Software for Big Science},
   publisher={Springer Science and Business Media LLC},
   author={Musella, Pasquale and Pandolfi, Francesco},
   year={2018},
   month={Nov},
   eprint={1805.00850},
   archivePrefix={arXiv},
   primaryClass={hep-ex}
}

@article{Bothmann,
    author = "Bothmann, Enrico and Debbio, Luigi",
    archivePrefix = "arXiv",
    doi = "10.1007/JHEP01(2019)033",
    eprint = "1808.07802",
    journal = "JHEP",
    pages = "033",
    primaryClass = "hep-ph",
    title = "{Reweighting a parton shower using a neural network: the final-state case}",
    volume = "01",
    year = "2019"
}

@article{Bothmann:2020ywa,
    author = "Bothmann, Enrico and Janßen, Timo and Knobbe, Max and Schmale, Tobias and Schumann, Steffen",
    archivePrefix = "arXiv",
    eprint = "2001.05478",
    month = "1",
    primaryClass = "hep-ph",
    reportNumber = "MCNET-20-02, MCNET-20-01",
    title = "{Exploring phase space with Neural Importance Sampling}",
    year = "2020"
}

@article{Monk,
    author = "Monk, J.W.",
    archivePrefix = "arXiv",
    doi = "10.1007/JHEP12(2018)021",
    eprint = "1807.03685",
    journal = "JHEP",
    pages = "021",
    primaryClass = "hep-ph",
    title = "{Deep Learning as a Parton Shower}",
    volume = "12",
    year = "2018"
}

@article{JUNIPR,
    author = "Andreassen, Anders and Feige, Ilya and Frye, Christopher and Schwartz, Matthew D.",
    archivePrefix = "arXiv",
    doi = "10.1140/epjc/s10052-019-6607-9",
    eprint = "1804.09720",
    journal = "Eur. Phys. J. C",
    number = "2",
    pages = "102",
    primaryClass = "hep-ph",
    title = "{JUNIPR: a Framework for Unsupervised Machine Learning in Particle Physics}",
    volume = "79",
    year = "2019"
}

@article{Klimek:2018mza,
    author = "Klimek, Matthew D. and Perelstein, Maxim",
    archivePrefix = "arXiv",
    eprint = "1810.11509",
    month = "10",
    primaryClass = "hep-ph",
    title = "{Neural Network-Based Approach to Phase Space Integration}",
    year = "2018"
}
@article{Bendavid:2017zhk,
    author = "Bendavid, Joshua",
    archivePrefix = "arXiv",
    eprint = "1707.00028",
    month = "6",
    primaryClass = "hep-ph",
    title = "{Efficient Monte Carlo Integration Using Boosted Decision Trees and Generative Deep Neural Networks}",
    year = "2017"
}

@article{Otten:2019hhl,
    author = "Otten, Sydney and others",
    archivePrefix = "arXiv",
    eprint = "1901.00875",
    month = "1",
    primaryClass = "hep-ph",
    title = "{Event Generation and Statistical Sampling for Physics with Deep Generative Models and a Density Information Buffer}",
    year = "2019"
}

@article{KaustuvGAN,
    author = "Hashemi, Bobak and Amin, Nick and Datta, Kaustuv and Olivito, Dominick and Pierini, Maurizio",
    archivePrefix = "arXiv",
    eprint = "1901.05282",
    month = "1",
    primaryClass = "hep-ex",
    title = "{LHC analysis-specific datasets with Generative Adversarial Networks}",
    year = "2019"
}

@article{DiJetGAN,
    author = "Di Sipio, Riccardo and Faucci Giannelli, Michele and Ketabchi Haghighat, Sana and Palazzo, Serena",
    archivePrefix = "arXiv",
    doi = "10.1007/JHEP08(2019)110",
    eprint = "1903.02433",
    journal = "JHEP",
    pages = "110",
    primaryClass = "hep-ex",
    title = "{DijetGAN: A Generative-Adversarial Network Approach for the Simulation of QCD Dijet Events at the LHC}",
    volume = "08",
    year = "2019"
}

@article{FlowGeneration,
    author = "Gao, Christina and Höche, Stefan and Isaacson, Joshua and Krause, Claudius and Schulz, Holger",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.101.076002",
    eprint = "2001.10028",
    journal = "Phys. Rev. D",
    number = "7",
    pages = "076002",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-20-009-SCD-T, MCNET-20-03",
    title = "{Event Generation with Normalizing Flows}",
    volume = "101",
    year = "2020"
}

@article{ButterSubtraction,
    author = "Butter, Anja and Plehn, Tilman and Winterhalder, Ramon",
    archivePrefix = "arXiv",
    eprint = "1912.08824",
    month = "12",
    primaryClass = "hep-ph",
    title = "{How to GAN Event Subtraction}",
    year = "2019"
}

@article{GANFolding,
    author = "Bellagente, Marco and Butter, Anja and Kasieczka, Gregor and Plehn, Tilman and Winterhalder, Ramon",
    archivePrefix = "arXiv",
    eprint = "1912.00477",
    month = "12",
    primaryClass = "hep-ph",
    title = "{How to GAN away Detector Effects}",
    year = "2019"
}

@article{LundCycleGAN,
    author = "Carrazza, Stefano and Dreyer, Frédéric A.",
    archivePrefix = "arXiv",
    doi = "10.1140/epjc/s10052-019-7501-1",
    eprint = "1909.01359",
    journal = "Eur. Phys. J. C",
    number = "11",
    pages = "979",
    primaryClass = "hep-ph",
    reportNumber = "OUTP-19-09P, TIF-UNIMI-2019-14",
    title = "{Lund jet images from generative and cycle-consistent adversarial networks}",
    volume = "79",
    year = "2019"
}

@inproceedings{KyleInference,
    author = "Brehmer, Johann and Cranmer, Kyle and Espejo, Irina and Kling, Felix and Louppe, Gilles and Pavez, Juan",
    archivePrefix = "arXiv",
    booktitle = "{19th International Workshop on Advanced Computing and Analysis Techniques in Physics Research}: {Empowering the revolution: Bringing Machine Learning to High Performance Computing}",
    eprint = "1906.01578",
    month = "6",
    primaryClass = "hep-ph",
    title = "{Effective LHC measurements with matrix elements and machine learning}",
    year = "2019"
}

@article{INFERNO,
    author = "De Castro, Pablo and Dorigo, Tommaso",
    archivePrefix = "arXiv",
    doi = "10.1016/j.cpc.2019.06.007",
    eprint = "1806.04743",
    journal = "Comput. Phys. Commun.",
    pages = "170--179",
    primaryClass = "stat.ML",
    title = "{INFERNO: Inference-Aware Neural Optimisation}",
    volume = "244",
    year = "2019"
}

@article{KyleFlow,
    title="{Flows for simultaneous manifold learning and density estimation}",
    author={Johann Brehmer and Kyle Cranmer},
    year={2020},
    eprint={2003.13913},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@article{SALAD,
    author = "Andreassen, Anders and Nachman, Benjamin and Shih, David",
    archivePrefix = "arXiv",
    eprint = "2001.05001",
    month = "1",
    primaryClass = "hep-ph",
    title = "{Simulation Assisted Likelihood-free Anomaly Detection}",
    year = "2020"
}

@article{layernorm,
    title="{Layer Normalization}",
    author="Jimmy Lei Ba and Jamie Ryan Kiros and Geoffrey E. Hinton",
    year={2016},
    eprint={1607.06450},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@article{SGD,
  title="{An overview of gradient descent optimization algorithms}",
  author={Ruder, Sebastian},
  year={2016},
  eprint={1609.04747},
  archivePrefix={arXiv}
} 


@inproceedings{ReLU,
author = {Nair, Vinod and Hinton, Geoffrey E.},
title = "{Rectified Linear Units Improve Restricted Boltzmann Machines}",
year = {2010},
isbn = {9781605589077},
address = {Madison, WI, USA},
booktitle = {Proceedings of the 27th International Conference on International Conference on Machine Learning},
pages = {807–814},
numpages = {8},
location = {Haifa, Israel},
series = {ICML’10}
}

@inproceedings{LReLU,
    author = {Andrew L. Maas and Awni Y. Hannun and Andrew Y. Ng},
    title = "{Rectifier nonlinearities improve neural network acoustic models}",
    booktitle = {Proceedings of ICML Workshop on Deep Learning for Audio, Speech and Language Processing},
    year = {2013}
}


@inproceedings{batchnorm,
    title="{Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift}",
    author={Sergey Ioffe and Christian Szegedy},
    year={2015},
    eprint={1502.03167},
    archivePrefix={arXiv},
    primaryClass={cs.LG},
    booktitle = 	 {Proceedings of the 32nd International Conference on Machine Learning},  
    pages = 	 {448--456},
    volume = 	 {37},
    address = 	 {Lille, France},
    month = 	 {07--09 Jul},
}

@article{ALAD,
    author = "Knapp, Oliver and Dissertori, Guenther and Cerri, Olmo and Nguyen, Thong Q. and Vlimant, Jean-Roch and Pierini, Maurizio",
    title = "{Adversarially Learned Anomaly Detection on CMS Open Data: re-discovering the top quark}",
    eprint = "2005.01598",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "5",
    year = "2020"
}

@article{ATLASAnomaly,
    author = "Aad, Georges and others",
    collaboration = "{ATLAS Collaboration}",
    title = "{Dijet resonance search with weak supervision using $\sqrt{s}=13$ TeV $pp$ collisions in the ATLAS detector}",
    eprint = "2005.02983",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "CERN-EP-2020-062",
    month = "5",
    year = "2020"
}
@article{SHiPGAN,
    author = "Ahdida, C. and others",
    collaboration = "SHiP",
    title = "{Fast simulation of muons produced at the SHiP experiment using Generative Adversarial Networks}",
    eprint = "1909.04451",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    doi = "10.1088/1748-0221/14/11/P11028",
    journal = "JINST",
    volume = "14",
    pages = "P11028",
    year = "2019"
}

@article{TaoNovelty,
    author = "Hajer, Jan and Li, Ying-Ying and Liu, Tao and Wang, He",
    title = "{Novelty Detection Meets Collider Physics}",
    eprint = "1807.10261",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.101.076015",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "7",
    pages = "076015",
    year = "2020"
}



